Classification with Conceptual Safeguards

We propose a new approach to promote safety in classification tasks with established concepts. Our approach -- called a conceptual safeguard -- acts as a verification layer for models that predict a target outcome by first predicting the presence of intermediate concepts. Given this architecture, a safeguard ensures that a model meets a minimal level of accuracy by abstaining from uncertain predictions. In contrast to a standard selective classifier, a safeguard provides an avenue to improve coverage by allowing a human to confirm the presence of uncertain concepts on instances on which it abstains. We develop methods to build safeguards that maximize coverage without compromising safety, namely techniques to propagate the uncertainty in concept predictions and to flag salient concepts for human review. We benchmark our approach on a collection of real-world and synthetic datasets, showing that it can improve performance and coverage in deep learning tasks.

==> ext/iclr2024/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> figures/2024/vjan/result_tables/coverage_threshold_budget0.1_multiclass.tex <==
\resizebox{\linewidth}{!}{
\centering\begingroup\fontsize{8}{10}\selectfont
\renewcommand{\predictionthresholds}[0]{\cell{l}{$\tau=0.05$\\ $\tau=0.1$\\ $\tau=0.15$\\ $\tau=0.2$}}
\begin{tabular}{llccccc}
Dataset & Prediction Thresholds & X->Y MLP & Baseline & CS & Baseline + RandomConf & CS + ImpactConf \\
\midrule
\cubtypesinfo & \predictionthresholds & \cell{r}{0.0\%\\ 43.6\%\\ 59.8\%\\ 74.0\%} & \cell{r}{3.3\%\\ 37.9\%\\ 48.4\%\\ 57.9\%} & \cell{r}{21.0\%\\ 29.9\%\\ 38.7\%\\ 50.1\%} & \cell{r}{16.7\%\\ 45.7\%\\ 58.3\%\\ 68.1\%} & \cell{r}{\cellcolor{fgood}68.95\%\\ \cellcolor{fgood}75.96\%\\ \cellcolor{fgood}83.81\%\\ \cellcolor{fgood}92.15\%} \\
\midrule
\end{tabular}
\endgroup{}
}


==> figures/2024/vjan/result_tables/coverage_threshold_budget0.2_multiclass.tex <==
\resizebox{\linewidth}{!}{
\centering\begingroup\fontsize{8}{10}\selectfont
\renewcommand{\predictionthresholds}[0]{\cell{l}{$\tau=0.05$\\ $\tau=0.1$\\ $\tau=0.15$\\ $\tau=0.2$}}
\begin{tabular}{llccccc}
Dataset & Prediction Thresholds & X->Y MLP & Baseline & CS & Baseline + RandomConf & CS + ImpactConf \\
\midrule
\cubtypesinfo & \predictionthresholds & \cell{r}{0.0\%\\ 43.6\%\\ 59.8\%\\ 74.0\%} & \cell{r}{3.3\%\\ 37.9\%\\ 48.4\%\\ 57.9\%} & \cell{r}{21.0\%\\ 29.9\%\\ 38.7\%\\ 50.1\%} & \cell{r}{3.7\%\\ 50.9\%\\ 64.1\%\\ 88.6\%} & \cell{r}{\cellcolor{fgood}77.30\%\\ \cellcolor{fgood}82.97\%\\ \cellcolor{fgood}100.00\%\\ \cellcolor{fgood}100.00\%} \\
\midrule
\end{tabular}
\endgroup{}
}


==> figures/2024/vjan/result_tables/coverage_threshold_budget0.5_multiclass.tex <==
\resizebox{\linewidth}{!}{
\centering\begingroup\fontsize{8}{10}\selectfont
\renewcommand{\predictionthresholds}[0]{\cell{l}{$\tau=0.05$\\ $\tau=0.1$\\ $\tau=0.15$\\ $\tau=0.2$}}
\begin{tabular}{llccccc}
Dataset & Prediction Thresholds & X->Y MLP & Baseline & CS & Baseline + RandomConf & CS + ImpactConf \\
\midrule
\cubtypesinfo & \predictionthresholds & \cell{r}{0.0\%\\ 43.6\%\\ 59.8\%\\ 74.0\%} & \cell{r}{3.3\%\\ 37.9\%\\ 48.4\%\\ 57.9\%} & \cell{r}{21.0\%\\ 29.9\%\\ 38.7\%\\ 50.1\%} & \cell{r}{71.8\%\\ 86.1\%\\ 91.5\%\\ \cellcolor{fgood}100.00\%} & \cell{r}{\cellcolor{fgood}92.99\%\\ \cellcolor{fgood}100.00\%\\ \cellcolor{fgood}100.00\%\\ \cellcolor{fgood}100.00\%} \\
\midrule
\end{tabular}
\endgroup{}
}


==> figures/cub/v0/int_budget_table_0.2.tex <==

\begin{table*}
    \centering
    \caption{Intervention Budget 0.2}
    \label{int_budget_table_0.2}
        \begin{tabular}{lrrlr}
\hline
 Strategy            &   total interventions &   accuracy & coverage   &   total wasted interventions \\
\hline
 UncertainProp + Int &                    12 &     0.6277 & 96.01\%    &                            9 \\
 Baseline            &                     0 &     0.6239 & 93.90\%    &                            0 \\
 UncertaintyProp     &                     0 &     0.624  & 94.77\%    &                            0 \\
 nan                 &                    10 &     0.6247 & 96.60\%    &                            8 \\
 nan                 &                     9 &     0.6237 & 97.10\%    &                            7 \\
\hline
\end{tabular}
\end{table*}


==> figures/cub/v0/int_budget_table_0.4.tex <==

\begin{table*}
    \centering
    \caption{Intervention Budget 0.4}
    \label{int_budget_table_0.4}
        \begin{tabular}{lrrlr}
\hline
 Strategy            &   total interventions &   accuracy & coverage   &   total wasted interventions \\
\hline
 UncertainProp + Int &                    25 &     0.628  & 96.40\%    &                           13 \\
 Baseline            &                     0 &     0.6239 & 93.90\%    &                            0 \\
 UncertaintyProp     &                     0 &     0.624  & 94.77\%    &                            0 \\
 nan                 &                    29 &     0.6282 & 96.22\%    &                           14 \\
 nan                 &                    19 &     0.6248 & 97.29\%    &                           13 \\
\hline
\end{tabular}
\end{table*}


==> figures/cub/v0/int_budget_table_0.6.tex <==

\begin{table*}
    \centering
    \caption{Intervention Budget 0.6}
    \label{int_budget_table_0.6}
        \begin{tabular}{lrrlr}
\hline
 Strategy            &   total interventions &   accuracy & coverage   &   total wasted interventions \\
\hline
 UncertainProp + Int &                    43 &     0.6315 & 96.80\%    &                           18 \\
 Baseline            &                     0 &     0.6239 & 93.90\%    &                            0 \\
 UncertaintyProp     &                     0 &     0.624  & 94.77\%    &                            0 \\
 nan                 &                    43 &     0.6306 & 96.86\%    &                           17 \\
 nan                 &                   197 &     0.6967 & 88.77\%    &                           79 \\
\hline
\end{tabular}
\end{table*}


==> figures/cub/v0/int_budget_table_0.8.tex <==

\begin{table*}
    \centering
    \caption{Intervention Budget 0.8}
    \label{int_budget_table_0.8}
        \begin{tabular}{lrrlr}
\hline
 Strategy            &   total interventions &   accuracy & coverage   &   total wasted interventions \\
\hline
 UncertainProp + Int &                    57 &     0.6322 & 97.36\%    &                           22 \\
 Baseline            &                     0 &     0.6239 & 93.90\%    &                            0 \\
 UncertaintyProp     &                     0 &     0.624  & 94.77\%    &                            0 \\
 nan                 &                    57 &     0.6316 & 97.35\%    &                           22 \\
 nan                 &                   256 &     0.7053 & 90.40\%    &                           93 \\
\hline
\end{tabular}
\end{table*}


==> figures/cub/v0/method_indepen.tex <==

\begin{table*}
    \centering
    \caption{Method indepen}
    \label{method_indepen}
        \begin{tabular}{lrrlr}
\hline
 intervention strategy        &   total interventions &   accuracy & coverage   &   total wasted interventions \\
\hline
 all abstentions intervention &                 21328 &     0.9578 & 99.92\%    &                           53 \\
 variance intervention        &                  9395 &     0.9567 & 96.99\%    &                          212 \\
 random intervention          &                  9395 &     0.9533 & 85.36\%    &                         2691 \\
 no intervention              &                     0 &     0.9483 & 68.21\%    &                            0 \\
\hline
\end{tabular}
\end{table*}


==> figures/cub/v0/method_independent.tex <==

\begin{table*}
    \centering
    \caption{Method independent}
    \label{method_independent}
        \begin{tabular}{lrrrlr}
\hline
 intervention strategy        &   total interventions &   accuracy &    AUC & coverage   &   total wasted interventions \\
\hline
 all abstentions intervention &                   527 &     0.75   & 0.815  & 85.71\%    &                          170 \\
 variance intervention        &                   263 &     0.7223 & 0.7547 & 73.57\%    &                          119 \\
 random intervention          &                   263 &     0.6988 & 0.7507 & 72.86\%    &                          139 \\
 no intervention              &                     0 &     0.6667 & 0.6908 & 55.71\%    &                            0 \\
\hline
\end{tabular}
\end{table*}


==> figures/cub/v0/method_independent_intervention_all_abstentions_intervention.tex <==

\begin{table*}
    \centering
    \caption{Method: independent, Intervention Strategy: all abstentions intervention}
    \label{method_independent_intervention_all_abstentions_intervention}
        \begin{tabular}{}
\hline
 method   & total interventions   & accuracy   & AUC   & coverage   & total wasted interventions   \\
\hline
\hline
\end{tabular}
\end{table*}


==> figures/cub/v0/method_independent_intervention_no_intervention.tex <==

\begin{table*}
    \centering
    \caption{Method: independent, Intervention Strategy: no intervention}
    \label{method_independent_intervention_no_intervention}
        \begin{tabular}{}
\hline
 method   & total interventions   & accuracy   & AUC   & coverage   & total wasted interventions   \\
\hline
\hline
\end{tabular}
\end{table*}


==> figures/cub/v0/method_independent_intervention_random_intervention.tex <==

\begin{table*}
    \centering
    \caption{Method: independent, Intervention Strategy: random intervention}
    \label{method_independent_intervention_random_intervention}
        \begin{tabular}{}
\hline
 method   & total interventions   & accuracy   & AUC   & coverage   & total wasted interventions   \\
\hline
\hline
\end{tabular}
\end{table*}


==> figures/cub/v0/method_independent_intervention_variance_intervention.tex <==

\begin{table*}
    \centering
    \caption{Method: independent, Intervention Strategy: variance intervention}
    \label{method_independent_intervention_variance_intervention}
        \begin{tabular}{}
\hline
 method   & total interventions   & accuracy   & AUC   & coverage   & total wasted interventions   \\
\hline
\hline
\end{tabular}
\end{table*}


==> figures/cub/v0/method_ours.tex <==

\begin{table*}
    \centering
    \caption{Method ours}
    \label{method_ours}
        \begin{tabular}{lrrrlr}
\hline
 intervention strategy        &   total interventions &   accuracy &    AUC & coverage   &   total wasted interventions \\
\hline
 all abstentions intervention &                   544 &     0.7667 & 0.8252 & 85.71\%    &                          170 \\
 variance intervention        &                   272 &     0.7341 & 0.7598 & 71.43\%    &                          130 \\
 random intervention          &                   272 &     0.7302 & 0.7713 & 73.93\%    &                          126 \\
 no intervention              &                     0 &     0.6842 & 0.7031 & 54.29\%    &                            0 \\
\hline
\end{tabular}
\end{table*}


==> figures/cub/v0/method_ours_intervention_all_abstentions_intervention.tex <==

\begin{table*}
    \centering
    \caption{Method: ours, Intervention Strategy: all abstentions intervention}
    \label{method_ours_intervention_all_abstentions_intervention}
        \begin{tabular}{}
\hline
 method   & total interventions   & accuracy   & AUC   & coverage   & total wasted interventions   \\
\hline
\hline
\end{tabular}
\end{table*}


==> figures/cub/v0/method_ours_intervention_no_intervention.tex <==

\begin{table*}
    \centering
    \caption{Method: ours, Intervention Strategy: no intervention}
    \label{method_ours_intervention_no_intervention}
        \begin{tabular}{}
\hline
 method   & total interventions   & accuracy   & AUC   & coverage   & total wasted interventions   \\
\hline
\hline
\end{tabular}
\end{table*}


==> figures/cub/v0/method_ours_intervention_random_intervention.tex <==

\begin{table*}
    \centering
    \caption{Method: ours, Intervention Strategy: random intervention}
    \label{method_ours_intervention_random_intervention}
        \begin{tabular}{}
\hline
 method   & total interventions   & accuracy   & AUC   & coverage   & total wasted interventions   \\
\hline
\hline
\end{tabular}
\end{table*}


==> figures/cub/v0/method_ours_intervention_variance_intervention.tex <==

\begin{table*}
    \centering
    \caption{Method: ours, Intervention Strategy: variance intervention}
    \label{method_ours_intervention_variance_intervention}
        \begin{tabular}{}
\hline
 method   & total interventions   & accuracy   & AUC   & coverage   & total wasted interventions   \\
\hline
\hline
\end{tabular}
\end{table*}


==> figures/cub/v0/method_propagation.tex <==

\begin{table*}
    \centering
    \caption{Method propagation}
    \label{method_propagation}
        \begin{tabular}{lrrlr}
\hline
 intervention strategy        &   total interventions &   accuracy & coverage   &   total wasted interventions \\
\hline
 all abstentions intervention &                 30818 &     0.9863 & 99.61\%    &                           47 \\
 variance intervention        &                 15890 &     0.9854 & 98.12\%    &                          208 \\
 random intervention          &                 15890 &     0.9841 & 81.15\%    &                         4100 \\
 no intervention              &                     0 &     0.9829 & 53.94\%    &                            0 \\
\hline
\end{tabular}
\end{table*}


==> figures/cub/v0/method_sequential.tex <==

\begin{table*}
    \centering
    \caption{Method sequential}
    \label{method_sequential}
        \begin{tabular}{lrrrlr}
\hline
 intervention strategy        &   total interventions &   accuracy &    AUC & coverage   &   total wasted interventions \\
\hline
 all abstentions intervention &                   255 &     0.6364 & 0.6217 & 94.29\%    &                           68 \\
 variance intervention        &                   128 &     0.6096 & 0.6123 & 87.86\%    &                           57 \\
 random intervention          &                   128 &     0.5897 & 0.587  & 89.64\%    &                           52 \\
 no intervention              &                     0 &     0.5818 & 0.5773 & 78.57\%    &                            0 \\
\hline
\end{tabular}
\end{table*}


==> figures/cub/v0/method_sequential_intervention_all_abstentions_intervention.tex <==

\begin{table*}
    \centering
    \caption{Method: sequential, Intervention Strategy: all abstentions intervention}
    \label{method_sequential_intervention_all_abstentions_intervention}
        \begin{tabular}{lrrrlr}
\hline
 method     &   total interventions &   accuracy &    AUC & coverage   &   total wasted interventions \\
\hline
 sequential &                   255 &     0.6364 & 0.6217 & 94.29\%    &                           68 \\
\hline
\end{tabular}
\end{table*}


==> figures/cub/v0/method_sequential_intervention_no_intervention.tex <==

\begin{table*}
    \centering
    \caption{Method: sequential, Intervention Strategy: no intervention}
    \label{method_sequential_intervention_no_intervention}
        \begin{tabular}{lrrrlr}
\hline
 method     &   total interventions &   accuracy &    AUC & coverage   &   total wasted interventions \\
\hline
 sequential &                     0 &     0.5818 & 0.5773 & 78.57\%    &                            0 \\
\hline
\end{tabular}
\end{table*}


==> figures/cub/v0/method_sequential_intervention_random_intervention.tex <==

\begin{table*}
    \centering
    \caption{Method: sequential, Intervention Strategy: random intervention}
    \label{method_sequential_intervention_random_intervention}
        \begin{tabular}{lrrrlr}
\hline
 method     &   total interventions &   accuracy &   AUC & coverage   &   total wasted interventions \\
\hline
 sequential &                   128 &     0.5897 & 0.587 & 89.64\%    &                           52 \\
\hline
\end{tabular}
\end{table*}


==> figures/cub/v0/method_sequential_intervention_variance_intervention.tex <==

\begin{table*}
    \centering
    \caption{Method: sequential, Intervention Strategy: variance intervention}
    \label{method_sequential_intervention_variance_intervention}
        \begin{tabular}{lrrrlr}
\hline
 method     &   total interventions &   accuracy &    AUC & coverage   &   total wasted interventions \\
\hline
 sequential &                   128 &     0.6096 & 0.6123 & 87.86\%    &                           57 \\
\hline
\end{tabular}
\end{table*}


==> figures/result_tables/coverage_threshold_budget0.1.tex <==
\resizebox{\linewidth}{!}{
\centering\begingroup\fontsize{8}{10}\selectfont
\renewcommand{\predictionthresholds}[0]{\cell{l}{$\tau=0.05$\\ $\tau=0.1$\\ $\tau=0.15$\\ $\tau=0.2$}}
\begin{tabular}{llcccc}
Dataset & Prediction Thresholds & Baseline & Baseline + RandomConf & CS + RandomConf & CS + ImpactConf \\
\midrule
\warblerinfo & \predictionthresholds & \cell{r}{17.3\%\\ 74.0\%\\ \cellcolor{fgood}100.00\%\\ \cellcolor{fgood}100.00\%} & \cell{r}{26.0\%\\ 86.7\%\\ 97.3\%\\ \cellcolor{fgood}100.00\%} & \cell{r}{\cellcolor{fgood}92.00\%\\ \cellcolor{fgood}100.00\%\\ \cellcolor{fgood}100.00\%\\ \cellcolor{fgood}100.00\%} & \cell{r}{85.3\%\\ \cellcolor{fgood}100.00\%\\ \cellcolor{fgood}100.00\%\\ \cellcolor{fgood}100.00\%} \\
\midrule
\flycatcherinfo & \predictionthresholds & \cell{r}{26.9\%\\ 44.2\%\\ 44.2\%\\ 57.7\%} & \cell{r}{38.5\%\\ 38.5\%\\ 38.5\%\\ 96.2\%} & \cell{r}{51.9\%\\ 51.9\%\\ 76.9\%\\ 96.2\%} & \cell{r}{\cellcolor{fgood}100.00\%\\ \cellcolor{fgood}100.00\%\\ \cellcolor{fgood}100.00\%\\ \cellcolor{fgood}100.00\%} \\
\midrule
\cubcommoninfo & \predictionthresholds & \cell{r}{2.2\%\\ 12.5\%\\ 22.4\%\\ 22.4\%} & \cell{r}{3.2\%\\ 15.7\%\\ 26.4\%\\ 26.4\%} & \cell{r}{10.2\%\\ 10.2\%\\ 39.1\%\\ 63.1\%} & \cell{r}{\cellcolor{fgood}21.70\%\\ \cellcolor{fgood}52.09\%\\ \cellcolor{fgood}71.62\%\\ \cellcolor{fgood}91.82\%} \\
\midrule
\cubrareinfo & \predictionthresholds & \cell{r}{0.0\%\\ 11.4\%\\ 11.4\%\\ 31.9\%} & \cell{r}{0.0\%\\ 13.7\%\\ 24.4\%\\ 39.6\%} & \cell{r}{2.8\%\\ 18.5\%\\ 18.5\%\\ 35.6\%} & \cell{r}{\cellcolor{fgood}32.72\%\\ \cellcolor{fgood}32.72\%\\ \cellcolor{fgood}68.61\%\\ \cellcolor{fgood}91.99\%} \\
\midrule
\melanomainfo & \predictionthresholds & \cell{r}{0.0\%\\ 0.0\%\\ 0.0\%\\ 18.6\%} & \cell{r}{4.3\%\\ 4.3\%\\ 21.4\%\\ 21.4\%} & \cell{r}{\cellcolor{fgood}11.43\%\\ 27.1\%\\ 27.1\%\\ 52.9\%} & \cell{r}{2.9\%\\ \cellcolor{fgood}64.29\%\\ \cellcolor{fgood}64.29\%\\ \cellcolor{fgood}100.00\%} \\
\midrule
\skincancerinfo & \predictionthresholds & \cell{r}{0.0\%\\ 0.0\%\\ 11.0\%\\ 11.0\%} & \cell{r}{0.0\%\\ 13.4\%\\ 13.4\%\\ 30.5\%} & \cell{r}{9.8\%\\ \cellcolor{fgood}25.61\%\\ \cellcolor{fgood}53.66\%\\ \cellcolor{fgood}100.00\%} & \cell{r}{\cellcolor{fgood}25.61\%\\ \cellcolor{fgood}25.61\%\\ 45.1\%\\ 95.1\%} \\
\midrule
\syntheticlowinfo{} & \predictionthresholds & \cell{r}{0.0\%\\ 32.3\%\\ 43.6\%\\ 80.4\%} & \cell{r}{0.0\%\\ 33.2\%\\ 44.8\%\\ \cellcolor{fgood}84.00\%} & \cell{r}{\cellcolor{fgood}2.12\%\\ 34.5\%\\ 49.2\%\\ 80.2\%} & \cell{r}{0.0\%\\ \cellcolor{fgood}39.77\%\\ \cellcolor{fgood}65.35\%\\ 82.7\%} \\
\midrule
\synthetichighinfo{} & \predictionthresholds & \cell{r}{0.0\%\\ 0.0\%\\ 0.0\%\\ 0.0\%} & \cell{r}{0.0\%\\ 0.0\%\\ 0.0\%\\ 0.0\%} & \cell{r}{0.0\%\\ \cellcolor{fgood}3.24\%\\ \cellcolor{fgood}3.24\%\\ \cellcolor{fgood}3.24\%} & \cell{r}{0.0\%\\ 0.0\%\\ 2.4\%\\ 2.4\%} \\
\midrule
\end{tabular}
\endgroup{}
}


==> figures/result_tables/coverage_threshold_budget0.1_multiclass.tex <==
\resizebox{\linewidth}{!}{
\centering\begingroup\fontsize{8}{10}\selectfont
\renewcommand{\predictionthresholds}[0]{\cell{l}{$\tau=0.05$\\ $\tau=0.1$\\ $\tau=0.15$\\ $\tau=0.2$}}
\begin{tabular}{llcccc}
Dataset & Prediction Thresholds & Baseline & Baseline + RandomConf & CS + RandomConf & CS + ImpactConf \\
\midrule
% \cubspeciesinfo & \predictionthresholds & \cell{r}{8.7\%\\ 8.7\%\\ 12.4\%\\ 16.7\%} & \cell{r}{10.9\%\\ 15.4\%\\ 19.2\%\\ 19.2\%} & \cell{r}{6.7\%\\ 9.7\%\\ 18.0\%\\ 18.0\%} & \cell{r}{\cellcolor{fgood}31.55\%\\ \cellcolor{fgood}42.07\%\\ \cellcolor{fgood}42.07\%\\ \cellcolor{fgood}52.59\%} \\
% \midrule
\cubtypesinfo & \predictionthresholds & \cell{r}{3.3\%\\ 37.9\%\\ 48.4\%\\ 57.9\%} & \cell{r}{16.7\%\\ 45.7\%\\ 58.3\%\\ 68.1\%} & \cell{r}{25.7\%\\ 36.7\%\\ 50.3\%\\ 63.8\%} & \cell{r}{\cellcolor{fgood}68.95\%\\ \cellcolor{fgood}75.96\%\\ \cellcolor{fgood}83.81\%\\ \cellcolor{fgood}92.15\%} \\
\midrule
\end{tabular}
\endgroup{}
}


==> figures/result_tables/coverage_threshold_budget0.2.tex <==
\resizebox{\linewidth}{!}{
\centering\begingroup\fontsize{8}{10}\selectfont
\renewcommand{\predictionthresholds}[0]{\cell{l}{$\tau=0.05$\\ $\tau=0.1$\\ $\tau=0.15$\\ $\tau=0.2$}}
\begin{tabular}{llcccc}
Dataset & Prediction Thresholds & Baseline & Baseline + RandomConf & CS + RandomConf & CS + ImpactConf \\
\midrule
\warblerinfo & \predictionthresholds & \cell{r}{17.3\%\\ 74.0\%\\ \cellcolor{fgood}100.00\%\\ \cellcolor{fgood}100.00\%} & \cell{r}{30.0\%\\ 89.3\%\\ \cellcolor{fgood}100.00\%\\ \cellcolor{fgood}100.00\%} & \cell{r}{\cellcolor{fgood}94.67\%\\ \cellcolor{fgood}100.00\%\\ \cellcolor{fgood}100.00\%\\ \cellcolor{fgood}100.00\%} & \cell{r}{90.0\%\\ \cellcolor{fgood}100.00\%\\ \cellcolor{fgood}100.00\%\\ \cellcolor{fgood}100.00\%} \\
\midrule
\flycatcherinfo & \predictionthresholds & \cell{r}{26.9\%\\ 44.2\%\\ 44.2\%\\ 57.7\%} & \cell{r}{46.2\%\\ 46.2\%\\ 65.4\%\\ \cellcolor{fgood}100.00\%} & \cell{r}{63.5\%\\ 63.5\%\\ 82.7\%\\ \cellcolor{fgood}100.00\%} & \cell{r}{\cellcolor{fgood}84.62\%\\ \cellcolor{fgood}100.00\%\\ \cellcolor{fgood}100.00\%\\ \cellcolor{fgood}100.00\%} \\
\midrule
\cubcommoninfo & \predictionthresholds & \cell{r}{2.2\%\\ 12.5\%\\ 22.4\%\\ 22.4\%} & \cell{r}{0.0\%\\ 16.0\%\\ 29.4\%\\ 29.4\%} & \cell{r}{11.7\%\\ 22.7\%\\ 42.2\%\\ 70.1\%} & \cell{r}{\cellcolor{fgood}35.23\%\\ \cellcolor{fgood}52.09\%\\ \cellcolor{fgood}100.00\%\\ \cellcolor{fgood}100.00\%} \\
\midrule
\cubrareinfo & \predictionthresholds & \cell{r}{0.0\%\\ 11.4\%\\ 11.4\%\\ 31.9\%} & \cell{r}{0.0\%\\ 15.0\%\\ 15.0\%\\ 43.1\%} & \cell{r}{8.5\%\\ 19.5\%\\ 19.5\%\\ 65.9\%} & \cell{r}{\cellcolor{fgood}33.56\%\\ \cellcolor{fgood}51.09\%\\ \cellcolor{fgood}70.12\%\\ \cellcolor{fgood}100.00\%} \\
\midrule
\melanomainfo & \predictionthresholds & \cell{r}{0.0\%\\ 0.0\%\\ 0.0\%\\ 18.6\%} & \cell{r}{8.6\%\\ 8.6\%\\ 41.4\%\\ 41.4\%} & \cell{r}{37.1\%\\ 37.1\%\\ 64.3\%\\ 64.3\%} & \cell{r}{\cellcolor{fgood}61.43\%\\ \cellcolor{fgood}68.57\%\\ \cellcolor{fgood}100.00\%\\ \cellcolor{fgood}100.00\%} \\
\midrule
\skincancerinfo & \predictionthresholds & \cell{r}{0.0\%\\ 0.0\%\\ 11.0\%\\ 11.0\%} & \cell{r}{7.3\%\\ 15.9\%\\ 25.6\%\\ 36.6\%} & \cell{r}{17.1\%\\ 17.1\%\\ 17.1\%\\ \cellcolor{fgood}100.00\%} & \cell{r}{\cellcolor{fgood}32.93\%\\ \cellcolor{fgood}54.88\%\\ \cellcolor{fgood}85.37\%\\ 85.4\%} \\
\midrule
\syntheticlowinfo{} & \predictionthresholds & \cell{r}{0.0\%\\ 32.3\%\\ 43.6\%\\ 80.4\%} & \cell{r}{0.0\%\\ 33.9\%\\ 45.8\%\\ 86.8\%} & \cell{r}{\cellcolor{fgood}4.32\%\\ 36.3\%\\ 54.6\%\\ 83.8\%} & \cell{r}{0.0\%\\ \cellcolor{fgood}44.66\%\\ \cellcolor{fgood}69.16\%\\ \cellcolor{fgood}93.31\%} \\
\midrule
\synthetichighinfo{} & \predictionthresholds & \cell{r}{0.0\%\\ 0.0\%\\ 0.0\%\\ 0.0\%} & \cell{r}{0.0\%\\ 0.0\%\\ 0.0\%\\ 0.0\%} & \cell{r}{\cellcolor{fgood}0.10\%\\ 6.4\%\\ 6.4\%\\ 6.4\%} & \cell{r}{0.0\%\\ \cellcolor{fgood}11.17\%\\ \cellcolor{fgood}11.17\%\\ \cellcolor{fgood}11.17\%} \\
\midrule
\end{tabular}
\endgroup{}
}


==> figures/result_tables/coverage_threshold_budget0.2_multiclass.tex <==
\resizebox{\linewidth}{!}{
\centering\begingroup\fontsize{8}{10}\selectfont
\renewcommand{\predictionthresholds}[0]{\cell{l}{$\tau=0.05$\\ $\tau=0.1$\\ $\tau=0.15$\\ $\tau=0.2$}}
\begin{tabular}{llcccc}
Dataset & Prediction Thresholds & Baseline & Baseline + RandomConf & CS + RandomConf & CS + ImpactConf \\
\midrule
\cubspeciesinfo & \predictionthresholds & \cell{r}{8.7\%\\ 8.7\%\\ 12.4\%\\ 16.7\%} & \cell{r}{13.4\%\\ 17.7\%\\ 23.2\%\\ 33.1\%} & \cell{r}{12.7\%\\ 24.4\%\\ 24.4\%\\ 39.6\%} & \cell{r}{\cellcolor{fgood}50.92\%\\ \cellcolor{fgood}58.10\%\\ \cellcolor{fgood}68.61\%\\ \cellcolor{fgood}68.61\%} \\
\midrule
\cubtypesinfo & \predictionthresholds & \cell{r}{3.3\%\\ 37.9\%\\ 48.4\%\\ 57.9\%} & \cell{r}{3.7\%\\ 50.9\%\\ 64.1\%\\ 88.6\%} & \cell{r}{44.7\%\\ 60.1\%\\ 74.0\%\\ 88.8\%} & \cell{r}{\cellcolor{fgood}77.30\%\\ \cellcolor{fgood}82.97\%\\ \cellcolor{fgood}100.00\%\\ \cellcolor{fgood}100.00\%} \\
\midrule
\end{tabular}
\endgroup{}
}


==> figures/result_tables/coverage_threshold_budget0.2_partial_datasets.tex <==
\resizebox{\linewidth}{!}{
\centering\begingroup\fontsize{8}{10}\selectfont
\renewcommand{\predictionthresholds}[0]{\cell{l}{$\tau=0.05$\\ $\tau=0.1$\\ $\tau=0.15$\\ $\tau=0.2$}}
\begin{tabular}{llcccc}
Dataset & Prediction Thresholds & Baseline & Baseline + RandomConf & CS + RandomConf & CS + ImpactConf \\
\midrule
\warblerinfo & \predictionthresholds & \cell{r}{17.3\%\\ 74.0\%\\ \cellcolor{fgood}100.00\%\\ \cellcolor{fgood}100.00\%} & \cell{r}{30.0\%\\ 89.3\%\\ \cellcolor{fgood}100.00\%\\ \cellcolor{fgood}100.00\%} & \cell{r}{\cellcolor{fgood}94.67\%\\ \cellcolor{fgood}100.00\%\\ \cellcolor{fgood}100.00\%\\ \cellcolor{fgood}100.00\%} & \cell{r}{90.0\%\\ \cellcolor{fgood}100.00\%\\ \cellcolor{fgood}100.00\%\\ \cellcolor{fgood}100.00\%} \\
\midrule
\flycatcherinfo & \predictionthresholds & \cell{r}{26.9\%\\ 44.2\%\\ 44.2\%\\ 57.7\%} & \cell{r}{46.2\%\\ 46.2\%\\ 65.4\%\\ \cellcolor{fgood}100.00\%} & \cell{r}{63.5\%\\ 63.5\%\\ 82.7\%\\ \cellcolor{fgood}100.00\%} & \cell{r}{\cellcolor{fgood}84.62\%\\ \cellcolor{fgood}100.00\%\\ \cellcolor{fgood}100.00\%\\ \cellcolor{fgood}100.00\%} \\
\midrule
\melanomainfo & \predictionthresholds & \cell{r}{0.0\%\\ 0.0\%\\ 0.0\%\\ 18.6\%} & \cell{r}{8.6\%\\ 8.6\%\\ 41.4\%\\ 41.4\%} & \cell{r}{37.1\%\\ 37.1\%\\ 64.3\%\\ 64.3\%} & \cell{r}{\cellcolor{fgood}61.43\%\\ \cellcolor{fgood}68.57\%\\ \cellcolor{fgood}100.00\%\\ \cellcolor{fgood}100.00\%} \\
\midrule
\skincancerinfo & \predictionthresholds & \cell{r}{0.0\%\\ 0.0\%\\ 11.0\%\\ 11.0\%} & \cell{r}{7.3\%\\ 15.9\%\\ 25.6\%\\ 36.6\%} & \cell{r}{17.1\%\\ 17.1\%\\ 17.1\%\\ \cellcolor{fgood}100.00\%} & \cell{r}{\cellcolor{fgood}32.93\%\\ \cellcolor{fgood}54.88\%\\ \cellcolor{fgood}85.37\%\\ 85.4\%} \\
\midrule
\syntheticlowinfo{} & \predictionthresholds & \cell{r}{0.0\%\\ 32.3\%\\ 43.6\%\\ 80.4\%} & \cell{r}{0.0\%\\ 33.9\%\\ 45.8\%\\ 86.8\%} & \cell{r}{\cellcolor{fgood}4.32\%\\ 36.3\%\\ 54.6\%\\ 83.8\%} & \cell{r}{0.0\%\\ \cellcolor{fgood}44.66\%\\ \cellcolor{fgood}69.16\%\\ \cellcolor{fgood}93.31\%} \\
\midrule
\synthetichighinfo{} & \predictionthresholds & \cell{r}{0.0\%\\ 0.0\%\\ 0.0\%\\ 0.0\%} & \cell{r}{0.0\%\\ 0.0\%\\ 0.0\%\\ 0.0\%} & \cell{r}{\cellcolor{fgood}0.10\%\\ 6.4\%\\ 6.4\%\\ 6.4\%} & \cell{r}{0.0\%\\ \cellcolor{fgood}11.17\%\\ \cellcolor{fgood}11.17\%\\ \cellcolor{fgood}11.17\%} \\
\midrule
\end{tabular}
\endgroup{}
}


==> figures/result_tables/coverage_threshold_budget0.5.tex <==
\resizebox{\linewidth}{!}{
\centering\begingroup\fontsize{8}{10}\selectfont
\renewcommand{\predictionthresholds}[0]{\cell{l}{$\tau=0.05$\\ $\tau=0.1$\\ $\tau=0.15$\\ $\tau=0.2$}}
\begin{tabular}{llcccc}
Dataset & Prediction Thresholds & Baseline & Baseline + RandomConf & CS + RandomConf & CS + ImpactConf \\
\midrule
\warblerinfo & \predictionthresholds & \cell{r}{17.3\%\\ 74.0\%\\ \cellcolor{fgood}100.00\%\\ \cellcolor{fgood}100.00\%} & \cell{r}{84.7\%\\ 93.3\%\\ \cellcolor{fgood}100.00\%\\ \cellcolor{fgood}100.00\%} & \cell{r}{83.3\%\\ \cellcolor{fgood}100.00\%\\ \cellcolor{fgood}100.00\%\\ \cellcolor{fgood}100.00\%} & \cell{r}{\cellcolor{fgood}86.67\%\\ 92.7\%\\ \cellcolor{fgood}100.00\%\\ \cellcolor{fgood}100.00\%} \\
\midrule
\flycatcherinfo & \predictionthresholds & \cell{r}{26.9\%\\ 44.2\%\\ 44.2\%\\ 57.7\%} & \cell{r}{67.3\%\\ 76.9\%\\ 90.4\%\\ \cellcolor{fgood}100.00\%} & \cell{r}{82.7\%\\ 86.5\%\\ \cellcolor{fgood}100.00\%\\ \cellcolor{fgood}100.00\%} & \cell{r}{\cellcolor{fgood}100.00\%\\ \cellcolor{fgood}100.00\%\\ \cellcolor{fgood}100.00\%\\ \cellcolor{fgood}100.00\%} \\
\midrule
\cubcommoninfo & \predictionthresholds & \cell{r}{2.2\%\\ 12.5\%\\ 22.4\%\\ 22.4\%} & \cell{r}{10.7\%\\ 19.7\%\\ 69.8\%\\ 80.8\%} & \cell{r}{17.0\%\\ 51.6\%\\ 81.0\%\\ 81.0\%} & \cell{r}{\cellcolor{fgood}100.00\%\\ \cellcolor{fgood}100.00\%\\ \cellcolor{fgood}100.00\%\\ \cellcolor{fgood}100.00\%} \\
\midrule
\cubrareinfo & \predictionthresholds & \cell{r}{0.0\%\\ 11.4\%\\ 11.4\%\\ 31.9\%} & \cell{r}{3.0\%\\ 18.5\%\\ 67.4\%\\ 67.4\%} & \cell{r}{14.5\%\\ 28.4\%\\ 77.5\%\\ 77.5\%} & \cell{r}{\cellcolor{fgood}100.00\%\\ \cellcolor{fgood}100.00\%\\ \cellcolor{fgood}100.00\%\\ \cellcolor{fgood}100.00\%} \\
\midrule
\melanomainfo & \predictionthresholds & \cell{r}{0.0\%\\ 0.0\%\\ 0.0\%\\ 18.6\%} & \cell{r}{18.6\%\\ 30.0\%\\ 51.4\%\\ 75.7\%} & \cell{r}{44.3\%\\ 62.9\%\\ \cellcolor{fgood}100.00\%\\ \cellcolor{fgood}100.00\%} & \cell{r}{\cellcolor{fgood}72.86\%\\ \cellcolor{fgood}80.00\%\\ \cellcolor{fgood}100.00\%\\ \cellcolor{fgood}100.00\%} \\
\midrule
\skincancerinfo & \predictionthresholds & \cell{r}{0.0\%\\ 0.0\%\\ 11.0\%\\ 11.0\%} & \cell{r}{0.0\%\\ 28.0\%\\ 56.1\%\\ 84.1\%} & \cell{r}{\cellcolor{fgood}30.49\%\\ 42.7\%\\ 85.4\%\\ 85.4\%} & \cell{r}{0.0\%\\ \cellcolor{fgood}48.78\%\\ \cellcolor{fgood}100.00\%\\ \cellcolor{fgood}100.00\%} \\
\midrule
\syntheticlowinfo{} & \predictionthresholds & \cell{r}{0.0\%\\ 32.3\%\\ 43.6\%\\ 80.4\%} & \cell{r}{0.0\%\\ 36.0\%\\ 65.6\%\\ 91.6\%} & \cell{r}{11.0\%\\ \cellcolor{fgood}41.99\%\\ 64.1\%\\ 92.8\%} & \cell{r}{\cellcolor{fgood}19.75\%\\ 38.7\%\\ \cellcolor{fgood}78.19\%\\ \cellcolor{fgood}100.00\%} \\
\midrule
\synthetichighinfo{} & \predictionthresholds & \cell{r}{0.0\%\\ 0.0\%\\ 0.0\%\\ 0.0\%} & \cell{r}{0.0\%\\ 0.0\%\\ 0.0\%\\ 0.0\%} & \cell{r}{\cellcolor{fgood}1.67\%\\ 15.8\%\\ 15.8\%\\ 15.8\%} & \cell{r}{0.0\%\\ \cellcolor{fgood}29.55\%\\ \cellcolor{fgood}29.55\%\\ \cellcolor{fgood}68.25\%} \\
\midrule
\end{tabular}
\endgroup{}
}


==> figures/result_tables/coverage_threshold_budget0.5_multiclass.tex <==
\resizebox{\linewidth}{!}{
\centering\begingroup\fontsize{8}{10}\selectfont
\renewcommand{\predictionthresholds}[0]{\cell{l}{$\tau=0.05$\\ $\tau=0.1$\\ $\tau=0.15$\\ $\tau=0.2$}}
\begin{tabular}{llcccc}
Dataset & Prediction Thresholds & Baseline & Baseline + RandomConf & CS + RandomConf & CS + ImpactConf \\
\midrule
\cubspeciesinfo & \predictionthresholds & \cell{r}{8.7\%\\ 8.7\%\\ 12.4\%\\ 16.7\%} & \cell{r}{37.1\%\\ 45.1\%\\ 55.9\%\\ 69.4\%} & \cell{r}{46.1\%\\ 55.9\%\\ 70.1\%\\ 70.1\%} & \cell{r}{\cellcolor{fgood}67.11\%\\ \cellcolor{fgood}76.79\%\\ \cellcolor{fgood}84.64\%\\ \cellcolor{fgood}100.00\%} \\
\midrule
\cubtypesinfo & \predictionthresholds & \cell{r}{3.3\%\\ 37.9\%\\ 48.4\%\\ 57.9\%} & \cell{r}{71.8\%\\ 86.1\%\\ 91.5\%\\ \cellcolor{fgood}100.00\%} & \cell{r}{72.5\%\\ 92.0\%\\ 99.8\%\\ \cellcolor{fgood}100.00\%} & \cell{r}{\cellcolor{fgood}92.99\%\\ \cellcolor{fgood}100.00\%\\ \cellcolor{fgood}100.00\%\\ \cellcolor{fgood}100.00\%} \\
\midrule
\end{tabular}
\endgroup{}
}


==> figures/sep2023/v0/interventions_performance_table.tex <==

\begin{table*}
    \centering
    \caption{}
    \label{interventions_performance_table}
        \begin{tabular}{lllrl}
\hline
 dataset   & Strategy                  & Interventions Performed   &   accuracy & coverage   \\
\hline
 Synth25%  & Baseline                  & 0%                        &     0.7576 & 100.00\%   \\
 Synth25%  & Baseline + RandVer        & 10%                       &     0.7638 & 100.00\%   \\
 Synth25%  & UncertainProp + RandVer   & 10%                       &     0.764  & 100.00\%   \\
 Synth25%  & UncertainProp + ImpactVer & 10%                       &     0.7792 & 100.00\%   \\
\hline
\end{tabular}
\end{table*}


==> figures/sep2023/v0/interventions_performance_table_cubbottom60.tex <==

\begin{table*}
    \centering
    \caption{}
    \label{interventions_performance_table}
        \begin{tabular}{lllll}
\hline
 dataset     & Strategy                  & Interventions   & Accuracy   & Coverage   \\
\hline
 CUBBottom60 & Baseline                  & 0\%             & 67.11\%    & 100\%      \\
 CUBBottom60 & Baseline + RandVer        & 10\%            & 65.78\%    & 100\%      \\
 CUBBottom60 & UncertainProp + RandVer   & 10\%            & 72.79\%    & 100\%      \\
 CUBBottom60 & UncertainProp + ImpactVer & 10\%            & 78.30\%    & 100\%      \\
\hline
\end{tabular}
\end{table*}


==> figures/sep2023/v0/interventions_performance_table_cubtop10.tex <==

\begin{table*}
    \centering
    \caption{}
    \label{interventions_performance_table}
        \begin{tabular}{lllll}
\hline
 dataset   & Strategy                  & Interventions   & Accuracy   & Coverage   \\
\hline
 CUBTop10  & Baseline                  & 0\%             & 66.94\%    & 100\%      \\
 CUBTop10  & Baseline + RandVer        & 10\%            & 67.11\%    & 100\%      \\
 CUBTop10  & UncertainProp + RandVer   & 10\%            & 73.46\%    & 100\%      \\
 CUBTop10  & UncertainProp + ImpactVer & 10\%            & 79.13\%    & 100\%      \\
\hline
\end{tabular}
\end{table*}


==> figures/sep2023/v0/interventions_performance_table_melanoma.tex <==

\begin{table*}
    \centering
    \caption{}
    \label{interventions_performance_table}
        \begin{tabular}{lllll}
\hline
 dataset   & Strategy                  & Interventions   & Accuracy   & Coverage   \\
\hline
 Melanoma  & Baseline                  & 0\%             & 57.14\%    & 100\%      \\
 Melanoma  & Baseline + RandVer        & 10\%            & 64.29\%    & 100\%      \\
 Melanoma  & UncertainProp + RandVer   & 10\%            & 74.29\%    & 100\%      \\
 Melanoma  & UncertainProp + ImpactVer & 10\%            & 84.29\%    & 100\%      \\
\hline
\end{tabular}
\end{table*}

==> figures/sep2023/v0/interventions_performance_table_skincancer.tex <==

\begin{table*}
    \centering
    \caption{}
    \label{interventions_performance_table}
        \begin{tabular}{lllll}
\hline
 dataset    & Strategy                  & Interventions   & Accuracy   & Coverage   \\
\hline
 SkinCancer & Baseline                  & 0\%             & 63.41\%    & 100\%      \\
 SkinCancer & Baseline + RandVer        & 10\%            & 59.76\%    & 100\%      \\
 SkinCancer & UncertainProp + RandVer   & 10\%            & 73.17\%    & 100\%      \\
 SkinCancer & UncertainProp + ImpactVer & 10\%            & 78.05\%    & 100\%      \\
\hline
\end{tabular}
\end{table*}


==> figures/sep2023/v0/interventions_performance_table_synth25.tex <==

\begin{table*}
    \centering
    \caption{}
    \label{interventions_performance_table}
        \begin{tabular}{lllll}
\hline
 dataset   & Strategy                  & Interventions   & Accuracy   & Coverage   \\
\hline
 Synth25\% & Baseline                  & 0\%             & 75.76\%    & 100\%      \\
 Synth25\% & Baseline + RandVer        & 10\%            & 76.38\%    & 100\%      \\
 Synth25\% & UncertainProp + RandVer   & 10\%            & 76.40\%    & 100\%      \\
 Synth25\% & UncertainProp + ImpactVer & 10\%            & 77.92\%    & 100\%      \\
\hline
\end{tabular}
\end{table*}


==> figures/sep2023/v0/perf_coverage_strategy.tex <==

\begin{table*}
    \centering
    \caption{}
    \label{perf_coverage_strategy}
        \begin{tabular}{lllrl}
\hline
 dataset   & Strategy                  & Interventions Performed   &   accuracy & coverage   \\
\hline
 Synth25%  & Baseline                  & 0%                        &     0.7576 & 100.00\%   \\
 Synth25%  & Baseline + RandVer        & 10%                       &     0.7638 & 100.00\%   \\
 Synth25%  & UncertainProp + RandVer   & 10%                       &     0.764  & 100.00\%   \\
 Synth25%  & UncertainProp + ImpactVer & 10%                       &     0.7792 & 100.00\%   \\
\hline
\end{tabular}
\end{table*}


==> figures/sep2023/v0/tables/overview_results.tex <==

    \begin{tabular}{m{0.15\textwidth}p{0.267\textwidth}p{0.267\textwidth}p{0.267\textwidth}} \hline
        \multicolumn{4}{c}{\includegraphics[width=\textwidth]{figures/sep2023/v0/tables/overview_results_legend.pdf}} \\ \hline
            \adjustbox{valign=c}{\parbox{0.15\textwidth}{\textds{CUBCommon}\\ n=5,994 \\ m=112 \\ \cite{cub}}} &
                \adjustbox{valign=c}{\includegraphics[width=0.267\textwidth]{figures/sep2023/v0/tables/subfigures/coverage_accuracy_CUBCommon_0.0.pdf}} &
                \adjustbox{valign=c}{\includegraphics[width=0.267\textwidth]{figures/sep2023/v0/tables/subfigures/coverage_accuracy_CUBCommon_0.1.pdf}} &
                \adjustbox{valign=c}{\includegraphics[width=0.267\textwidth]{figures/sep2023/v0/tables/subfigures/coverage_accuracy_CUBCommon_0.8.pdf}}  \\ 
            \hline
            \adjustbox{valign=c}{\parbox{0.15\textwidth}{\textds{CUBRare}\\ n=5,994 \\ m=112 \\ \cite{cub}}} &
                \adjustbox{valign=c}{\includegraphics[width=0.267\textwidth]{figures/sep2023/v0/tables/subfigures/coverage_accuracy_CUBRare_0.0.pdf}} &
                \adjustbox{valign=c}{\includegraphics[width=0.267\textwidth]{figures/sep2023/v0/tables/subfigures/coverage_accuracy_CUBRare_0.1.pdf}} &
                \adjustbox{valign=c}{\includegraphics[width=0.267\textwidth]{figures/sep2023/v0/tables/subfigures/coverage_accuracy_CUBRare_0.8.pdf}}  \\ 
            \hline
            \adjustbox{valign=c}{\parbox{0.15\textwidth}{\textds{Melanoma}\\ n=616 \\ m=17 \\ \cite{derm7pt}}} &
                \adjustbox{valign=c}{\includegraphics[width=0.267\textwidth]{figures/sep2023/v0/tables/subfigures/coverage_accuracy_Melanoma_0.0.pdf}} &
                \adjustbox{valign=c}{\includegraphics[width=0.267\textwidth]{figures/sep2023/v0/tables/subfigures/coverage_accuracy_Melanoma_0.1.pdf}} &
                \adjustbox{valign=c}{\includegraphics[width=0.267\textwidth]{figures/sep2023/v0/tables/subfigures/coverage_accuracy_Melanoma_0.8.pdf}}  \\ 
            \hline
            \adjustbox{valign=c}{\parbox{0.15\textwidth}{\textds{SkinCancer}\\ n=616 \\ m=17 \\ \cite{derm7pt}}} &
                \adjustbox{valign=c}{\includegraphics[width=0.267\textwidth]{figures/sep2023/v0/tables/subfigures/coverage_accuracy_SkinCancer_0.0.pdf}} &
                \adjustbox{valign=c}{\includegraphics[width=0.267\textwidth]{figures/sep2023/v0/tables/subfigures/coverage_accuracy_SkinCancer_0.1.pdf}} &
                \adjustbox{valign=c}{\includegraphics[width=0.267\textwidth]{figures/sep2023/v0/tables/subfigures/coverage_accuracy_SkinCancer_0.8.pdf}}  \\ 
            \hline
            \adjustbox{valign=c}{\parbox{0.15\textwidth}{\textds{Synth25}\\ n=100,000 \\ m=3 \\ }} &
                \adjustbox{valign=c}{\includegraphics[width=0.267\textwidth]{figures/sep2023/v0/tables/subfigures/coverage_accuracy_Synth25_0.0.pdf}} &
                \adjustbox{valign=c}{\includegraphics[width=0.267\textwidth]{figures/sep2023/v0/tables/subfigures/coverage_accuracy_Synth25_0.1.pdf}} &
                \adjustbox{valign=c}{\includegraphics[width=0.267\textwidth]{figures/sep2023/v0/tables/subfigures/coverage_accuracy_Synth25_0.8.pdf}} 
      \end{tabular}
    
    

==> figures/sep2023/v0/tables/overview_results_hardcopy.tex <==
\begin{tabular}{m{0.15\textwidth}p{0.26\textwidth}p{0.26\textwidth}p{0.26\textwidth}} \hline
        \multicolumn{4}{c}{\includegraphics[width=\textwidth]{figures/sep2023/v0/tables/overview_results_legend.pdf}} \\ \hline
            \adjustbox{valign=c}{\parbox{0.15\textwidth}{\textds{CUBCommon}\\ n=5,994 \\ m=112 \\ \cite{cub}}} &
                \adjustbox{valign=c}{\includegraphics[width=0.26\textwidth]{figures/sep2023/v0/tables/subfigures/coverage_accuracy_CUBCommon_0.0.pdf}} &
                \adjustbox{valign=c}{\includegraphics[width=0.26\textwidth]{figures/sep2023/v0/tables/subfigures/coverage_accuracy_CUBCommon_0.1.pdf}} &
                \adjustbox{valign=c}{\includegraphics[width=0.26\textwidth]{figures/sep2023/v0/tables/subfigures/coverage_accuracy_CUBCommon_0.8.pdf}}  \\ 
            \hline
            \adjustbox{valign=c}{\parbox{0.2\textwidth}{\textds{CUBRare}\\ n=5,994 \\ m=112 \\ \cite{cub}}} &
                \adjustbox{valign=c}{\includegraphics[width=0.26\textwidth]{figures/sep2023/v0/tables/subfigures/coverage_accuracy_CUBRare_0.0.pdf}} &
                \adjustbox{valign=c}{\includegraphics[width=0.26\textwidth]{figures/sep2023/v0/tables/subfigures/coverage_accuracy_CUBRare_0.1.pdf}} &
                \adjustbox{valign=c}{\includegraphics[width=0.26\textwidth]{figures/sep2023/v0/tables/subfigures/coverage_accuracy_CUBRare_0.8.pdf}}  \\ 
            \hline
            \adjustbox{valign=c}{\parbox{0.2\textwidth}{\textds{Melanoma}\\ n=616 \\ m=17 \\ \cite{derm7pt}}} &
                \adjustbox{valign=c}{\includegraphics[width=0.26\textwidth]{figures/sep2023/v0/tables/subfigures/coverage_accuracy_Melanoma_0.0.pdf}} &
                \adjustbox{valign=c}{\includegraphics[width=0.26\textwidth]{figures/sep2023/v0/tables/subfigures/coverage_accuracy_Melanoma_0.1.pdf}} &
                \adjustbox{valign=c}{\includegraphics[width=0.26\textwidth]{figures/sep2023/v0/tables/subfigures/coverage_accuracy_Melanoma_0.8.pdf}}  \\ 
            \hline
            \adjustbox{valign=c}{\parbox{0.2\textwidth}{\textds{SkinCancer}\\ n=616 \\ m=17 \\ \cite{derm7pt}}} &
                \adjustbox{valign=c}{\includegraphics[width=0.26\textwidth]{figures/sep2023/v0/tables/subfigures/coverage_accuracy_SkinCancer_0.0.pdf}} &
                \adjustbox{valign=c}{\includegraphics[width=0.26\textwidth]{figures/sep2023/v0/tables/subfigures/coverage_accuracy_SkinCancer_0.1.pdf}} &
                \adjustbox{valign=c}{\includegraphics[width=0.26\textwidth]{figures/sep2023/v0/tables/subfigures/coverage_accuracy_SkinCancer_0.8.pdf}}  \\ 
            \hline
            \adjustbox{valign=c}{\parbox{0.2\textwidth}{\textds{Synth25}\\ n=100,000 \\ m=112 \\ NA}} &
                \adjustbox{valign=c}{\includegraphics[width=0.26\textwidth]{figures/sep2023/v0/tables/subfigures/coverage_accuracy_Synth25_0.0.pdf}} &
                \adjustbox{valign=c}{\includegraphics[width=0.26\textwidth]{figures/sep2023/v0/tables/subfigures/coverage_accuracy_Synth25_0.1.pdf}} &
                \adjustbox{valign=c}{\includegraphics[width=0.26\textwidth]{figures/sep2023/v0/tables/subfigures/coverage_accuracy_Synth25_0.8.pdf}} 
      \end{tabular}

==> figures/synth_data_results/strats_v11/int_budget_table_0.0.tex <==

\begin{table*}
    \centering
    \caption{Intervention Budget 0.0}
    \label{int_budget_table_0.0}
        \begin{tabular}{lrrlr}
\hline
 intervention strategy        &   total interventions &   accuracy & coverage   &   total wasted interventions \\
\hline
 all abstentions intervention &                 34696 &     0.8384 & 64.37\%    &                        21375 \\
 variance intervention        &                     0 &     0.7799 & 42.17\%    &                            0 \\
 random intervention          &                     0 &     0.7799 & 42.17\%    &                            0 \\
 no intervention              &                     0 &     0.7799 & 42.17\%    &                            0 \\
\hline
\end{tabular}
\end{table*}


==> figures/synth_data_results/strats_v11/int_budget_table_0.2.tex <==

\begin{table*}
    \centering
    \caption{Intervention Budget 0.2}
    \label{int_budget_table_0.2}
        \begin{tabular}{lrrlr}
\hline
 intervention strategy        &   total interventions &   accuracy & coverage   &   total wasted interventions \\
\hline
 all abstentions intervention &                 34696 &     0.8384 & 64.37\%    &                        21375 \\
 variance intervention        &                  6939 &     0.8067 & 52.05\%    &                         4932 \\
 random intervention          &                  6939 &     0.8217 & 47.98\%    &                         5383 \\
 no intervention              &                     0 &     0.7799 & 42.17\%    &                            0 \\
\hline
\end{tabular}
\end{table*}


==> figures/synth_data_results/strats_v11/int_budget_table_0.4.tex <==

\begin{table*}
    \centering
    \caption{Intervention Budget 0.4}
    \label{int_budget_table_0.4}
        \begin{tabular}{lrrlr}
\hline
 intervention strategy        &   total interventions &   accuracy & coverage   &   total wasted interventions \\
\hline
 all abstentions intervention &                 34696 &     0.8384 & 64.37\%    &                        21375 \\
 variance intervention        &                 13878 &     0.8256 & 59.69\%    &                         9622 \\
 random intervention          &                 13878 &     0.8251 & 52.95\%    &                        10189 \\
 no intervention              &                     0 &     0.7799 & 42.17\%    &                            0 \\
\hline
\end{tabular}
\end{table*}


==> figures/synth_data_results/strats_v11/int_budget_table_0.6.tex <==

\begin{table*}
    \centering
    \caption{Intervention Budget 0.6}
    \label{int_budget_table_0.6}
        \begin{tabular}{lrrlr}
\hline
 intervention strategy        &   total interventions &   accuracy & coverage   &   total wasted interventions \\
\hline
 all abstentions intervention &                 34696 &     0.8384 & 64.37\%    &                        21375 \\
 variance intervention        &                 20817 &     0.8318 & 64.11\%    &                        13224 \\
 random intervention          &                 20817 &     0.8285 & 57.26\%    &                        14426 \\
 no intervention              &                     0 &     0.7799 & 42.17\%    &                            0 \\
\hline
\end{tabular}
\end{table*}


==> figures/synth_data_results/strats_v11/int_budget_table_0.8.tex <==

\begin{table*}
    \centering
    \caption{Intervention Budget 0.8}
    \label{int_budget_table_0.8}
        \begin{tabular}{lrrlr}
\hline
 intervention strategy        &   total interventions &   accuracy & coverage   &   total wasted interventions \\
\hline
 all abstentions intervention &                 34696 &     0.8384 & 64.37\%    &                        21375 \\
 variance intervention        &                 27757 &     0.8355 & 64.43\%    &                        17534 \\
 random intervention          &                 27757 &     0.8335 & 61.05\%    &                        18135 \\
 no intervention              &                     0 &     0.7799 & 42.17\%    &                            0 \\
\hline
\end{tabular}
\end{table*}


==> figures/synth_data_results/strats_v11/int_budget_table_1.0.tex <==

\begin{table*}
    \centering
    \caption{Intervention Budget 1.0}
    \label{int_budget_table_1.0}
        \begin{tabular}{lrrlr}
\hline
 intervention strategy        &   total interventions &   accuracy & coverage   &   total wasted interventions \\
\hline
 all abstentions intervention &                 34696 &     0.8384 & 64.37\%    &                        21375 \\
 variance intervention        &                 34696 &     0.8384 & 64.37\%    &                        21375 \\
 random intervention          &                 34696 &     0.8384 & 64.37\%    &                        21375 \\
 no intervention              &                     0 &     0.7799 & 42.17\%    &                            0 \\
\hline
\end{tabular}
\end{table*}


==> notes.tex <==

\iftoggle{workingversion}{
\clearpage
}{
}
\subsection{Multiple Models}

One potential way to alleviate the distribution shift challenge is to train models on subsets of features. In this approach, a pool of models is constructed by considering different subsets of concepts. At inference time, the concepts for a sample are predicted, some of which may be missing, yielding a concept vector $c_s$. The concept vector $c_s$ is matched to a model $\hat{f}_s$ based on the subset of concepts $s$ that are present. One potential problem is scaling, as the number of subsets of concepts scales exponentially. To handle this, the pool of models could be constructed by considering only subsets that would lead to prediction performance above a certain threshold. That said, determining a priori which subsets would meet this criteria remains difficult. Another challenge is reliably measuring the performance of the overall system and implementing selective classification at the system (in addition to the concept) level. To understand this, imagine we measure performance for each model in the pool across all samples in the training data. However, the model will be used only on biased sample at inference time, since we hope to operate in the MNAR (Missing Not at Random) regime. Thus the estimated performance of each model (and hence the overall system) will be unreliable. 

\paragraph{How do we know that a concept has been detected with high uncertainty?}

\paragraph{How do we abstain from prediction in the front end / point users towards intervention?}

\paragraph{How do we measure the value of detecting the missing concepts?}

\paragraph{What is the training requirement}

\paragraph{What are potential caveats}



\subsection{Synthetic Data for Uncertainty Estimation}
\todo[]{Write down synthetic dataset here}


\begin{itemize}
    \item Bayesian Uncertainty Quantification with Synthetic Data \cite{phan2019bayesian}: Explores uncertainty with a BNN with dropout using a dataset of images with varying levels of "rain", "clouds", "puddles" and occlusion. Some helpful notation from this paper:
    
    
    
    Predictive Entropy captures the total amount of uncertainty (epistemic and aleatoric) and is equal to the sum of mutual information and aleatoric entropy. It is calculated as an entropy of the mean categorical distribution:
$$
\begin{aligned}
\mathbb{H}(\hat{\mathbf{y}} \mid \hat{\xb}) &=\mathbb{M I I}(\hat{\mathbf{y}} \mid \hat{\xb})+\mathbb{A} \mathbb{E}(\hat{\mathbf{y}} \mid \hat{\xb}) \\
&=-\sum_k p(\hat{\mathbf{y}}=k \mid \hat{\xb}) \log p(\hat{\mathbf{y}}=k \mid \hat{\xb})
\end{aligned}
$$
Aleatoric Entropy captures the aleatoric uncertainty and is calculated by averaging the entropy of each sampled categorical distribution.
$$
\mathbb{A} \mathbb{E}(\hat{\mathbf{y}} \mid \hat{\xb})=-\frac{1}{T} \sum_{k, i} p\left(\hat{\mathbf{y}}=k \mid \hat{\xb}, \omega_i\right) \log p\left(\hat{\mathbf{y}}=k \mid \hat{\xb}, \omega_i\right)
$$
Mutual Information captures the epistemic uncertainty and is calculated as:
$$
\mathbb{M}(\hat{\mathbf{y}} \mid \hat{\xb})=\mathbb{H}(\hat{\mathbf{y}} \mid \hat{\xb})-\mathbb{A} \mathbb{E}(\hat{\mathbf{y}} \mid \hat{\xb})
$$

\end{itemize}



\section{Related Work}

\subsection{Selective Classification}
\begin{itemize}

\item \cite{geifman2017selective}: Considers risk and abstention rate tradeoff 
$$
(f, g)(x) \triangleq \begin{cases}f(x), & \text { if } g(x)=1 \\ \text { don't know, } & \text { if } g(x)=0\end{cases}
$$

where $f$ is a classifier, $g$ is the rejector and $x$ is the input.

They consider risk with coverage $\phi$
$$
R(f, g) \triangleq \frac{E_P[\ell(f(x), y) g(x)]}{\phi(f, g)}
$$
\item \cite{el2010foundations}: trades off the abstention rate with accuracy (calls this "Risk-Coverage Trade-off."). Uses notation 
    $$
    (f, g)(x) \triangleq \begin{cases}\text { reject, }, & \text { w.p. } 1-g(x) \\ f(x), & \text { w.p. } g(x)\end{cases}
    $$
where $f$ is the base classifier, and $g$ is a selection function. If $g: X \rightarrow \{0,1\}$ then $g$ is deterministic, but abstention can also happen with some probability $[0,1]$, in which case $g$ is randomized. They use $\Phi(f, g) \triangleq \mathbf{E}[g(X)]$ for coverage and $R(f, g) \triangleq \frac{\mathbf{E}[\ell(f(X), Y) \cdot g(X)]}{\Phi(f, g)}$ for risk.
\item \cite{chow1970optimum}: The original selective classification paper. Introduced ``Chow's Rule'', a competitive baseline in which a sample is rejected if the confidence is lower than the cost of rejection (predict when one is $1-c$ confident): 

$$
f^*(\boldsymbol{x})= \begin{cases}{ }^{\abstain} & \max _y \eta_y(\boldsymbol{x}) \leq 1-c \\ \arg \max _y \eta_y(\boldsymbol{x}) & \text { otherwise }\end{cases}
$$
Here $f$ is the function that can yield $Y \cup \{\abstain\}$ and $\eta_y(x)$ is the probability of class $y$ given $x$, and $c$ is the cost of abstention.
\item \cite{mozannar2020consistent}: Proposed a consistent loss ($\hat{\theta} \rightarrow \theta^*$ as $n \rightarrow \infty$) for multiclass selective classification using connections with cost sensitive learning (e.g,. false negatives worse than false positives). References prior work that handles this problem for binary classification and  is applicable to the situation where the rejection cost can be
different for each x. They consider a split loss for when the model predicts vs when the expert predicts: 

$$
\begin{aligned}
L(h, r) & =\mathbb{E}_{(x, y) \sim \mathbf{P}, m \sim M \mid(x, y)}[\underbrace{l(x, y, h(x))}_{\text {classifier cost }} \underbrace{\mathbb{I}_{r(X)=0}}_{\text {predict }} \\
& +\overbrace{l_{\exp }(x, y, m)}^{\text {expert cost }} \overbrace{\mathbb{I}_{r(x)=1}}^{\text {defer }}]
\end{aligned}
$$

The propose the following surrogate loss, using cross entropy loss and cost sensitive learning:

$$
\begin{aligned}
& \widetilde{L}_{C E}\left(g_1, \cdots, g_{K+1}, x, c(1), \cdots, c(K+1)\right)= \\
& -\sum_{i=1}^{K+1}\left(\max _{j \in[K+1]} c(j)-c(i)\right) \log \left(\frac{\exp \left(g_i(x)\right)}{\sum_k \exp \left(g_k(x)\right)}\right)
\end{aligned}
$$

\item \cite{bartlett2008classification}: Proposes a surrogate loss to solve the problem of selective classification. They use notation: 

$$
\ell_{d, \delta}(z)= \begin{cases}1 & \text { if } z<-\delta \\ d & \text { if }|z| \leq \delta \\ 0 & \text { otherwise }\end{cases}
$$

where $\delta$ is the confidence threshold, $d$ is the cost of rejection, $z$ is the decision function. 

They reformulate this as a continuous surrogate loss: 

$$
\phi_d(z)= \begin{cases}1-a z & \text { if } z<0 \\ 1-z & \text { if } 0 \leq z<1 \\ 0 & \text { otherwise }\end{cases}
$$

\item \cite{cortes2016learning}: proposes learning two functions: a classifier $h$ and a rejection function $r$, and analyzes
the approach, giving a kernel-based algorithm in the binary setting. 

$$
R(h, r)=\underset{(x, y) \sim \mathcal{D}}{\mathbb{E}}\left[1_{y h(x) \leq 0} 1_{r(x)>0}+c 1_{r(x) \leq 0}\right]
$$

\item \cite{charoenphakdee2021classification}
Also uses connections to cost-sensitive learning, and seeks a method to reject without calculating posterior class probabilities. Considers 0-1 loss with a cost of rejection:

$$
\ell_{01 c}(f(\boldsymbol{x}), y)= \begin{cases}c & f(\boldsymbol{x})=® \\ \ell_{01}(f(\boldsymbol{x}), y) & \text { otherwise }\end{cases}
$$


\item \cite{fisch2022calibrated}: Aims to develop a new approach to selective
classification in which we propose a method for rejecting examples with “uncertain” uncertainties, using a separate selector network is trained to improve the
selective calibration error of a given base model including on OOD samples. The model is $f$, and the rejector is $g$, with loss function $\mathcal{L}$ and coverage $\psi$.

$$
(f, g)(x):= \begin{cases}f(x) & \text { if } g(x)=1 \\ \text { "abstain" } & \text { otherwise. }\end{cases}
$$

\begin{align*}
\mathcal{R}(f, g ; P) &:= \mathbb{E}[\mathcal{L}(f(X), Y) \mid g(X)=1] \\
&= \frac{\mathbb{E}[\mathcal{L}(f(X), Y) g(X)]}{\psi(f, g ; P)}
\end{align*}

\item \cite{wilder2020learning}:
End-to-end joint learning for human-AI teamwork, electing some examples to be sent to an expert and others to model. Learns a model with the mixtures
of expert loss and explores training jointly and separately.

\item \cite{narasimhan2022post}: Shows that existing selective classification losses can underfit when there's a non-trivial deferral cost and proposes post-hoc estimators that fit a deferral function on top of a base model with threshold correction. 




\end{itemize}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=.5\textwidth]{figures/aleatoric_epistemic.png}
%     \caption{The irreducible uncertainty in data that gives rise to uncertainty in predictions is aleatoric uncertainty (also known as data uncertainty). This type of uncertainty is not a property of the model, but rather is an inherent property of the data distribution, and hence, it is irreducible. In contrast, epistemic uncertainty (also known as knowledge uncertainty) occurs due to inadequate knowledge. One can define models to answer different questions in model-based prediction. For data-rich problems, there may be massive collections of data that are information poor. In such cases, AI-based methods can be used to define the efficient models that characterize the emergent features of the data. Very often, the data in hand are incomplete, noisy, discordant or multimodal}
%     \label{fig:aleatoric_epistemic}
% \end{figure}




\subsection{Concept Bottleneck Models}
\begin{itemize}

\item \cite{chauhan2022interactive}: Combines concept prediction uncertainty and influence to choose with the goal of 
maximally improving the final prediction. Uses a greedy algorithm to intervene on concepts up to a budget $B$.


\begin{algorithm}
\caption{Policy Rollout}
\label{algo:policy_rollout}
\begin{algorithmic}[1]
\REQUIRE $B$, $q_i$, $x$
\ENSURE Prediction $\operatorname{argmax}_{y \in \mathcal{Y}} p_\phi(c_S, p_\theta(c_{\bar{S}} \mid x))$
\STATE $S \gets \emptyset$
\STATE $b \gets 0$
\WHILE{$b \leq B$}
    \STATE $i \gets \psi(S)$
    \IF{$b \leq B-q_i$}
        \STATE Acquire the label for concept $c_i$
        \STATE $S \gets S \cup \{i\}$
        \STATE $b \gets b+q_i$
    \ELSE
        \STATE $b \gets B+1$
    \ENDIF
\ENDWHILE
\STATE Output prediction $\operatorname{argmax}_{y \in \mathcal{Y}} p_\phi(c_S, p_\theta(c_{\bar{S}} \mid x))$
\end{algorithmic}
\end{algorithm}

The interventions are determined by simply scoring the uncertainty and the concept importance: 

\begin{algorithm}
\caption{CooP policy}
\label{algo:coop_policy}
\begin{algorithmic}[1]
\STATE \textbf{Given} $p_\theta$, $p_\phi$, $q$, set of concepts acquired so far $S$, highest scoring predicted label based on acquired concepts $k \in \mathcal{Y}$, and score importance weights $\alpha$, $\beta$, $\gamma \in \mathbb{R}_+$.
\FORALL{$i \in \bar{S}$}
    \STATE Compute score$_i = \alpha \operatorname{CPU}(c_i ; S) + \beta \operatorname{CIS}(c_i ; S, k) - \gamma q_i$
\ENDFOR
\STATE \textbf{Output} $\operatorname{argmax}_i$ score$_i$
\end{algorithmic}
\end{algorithm}






\item Concept Bottlenecks \citet{koh2020concept}: Concept bottlenecks can be useful for understanding which important features the model might have learned (“Did the model deem the space between the knee joints too narrow?”) as well as for improving performance through concept correction (“If the radiologist informed the model the x-ray shows a bone spur, would its prediction change?”). They present weak evidence that CBMs require less data for similar performance and may be more robust to covariate shift.

\item Do Concept Bottleneck Models Learn as Intended? \citet{cbm_work}: The authors claim that of the three proposed training methods (independent, joint, and sequential), only the independent method may be able to achieve interpretability (which concepts are important), predictability (predict targets from concepts alone), and intervenability (fix concepts to improve performance). First, they use an ablation study to demonstrate that the joint model is learning labels before the concept to label component. This finding means that there's not a clear relationship between concepts and labels and that it may not be possible to predict labels from concepts alone. Second, They use Integrated Gradients, Gradient, and SmoothGrad to demonstrate that the model may be using other parts of the image to learn concepts (using the whole bird to learn wing color). Note: This experiment is perhaps poorly motivated since even humans use other parts of an image for concept learning (e.g., it can be difficult to determine if you're looking at a wing without looking at the rest of the image) and the examples were cherry-picked. 

\item Is Disentanglement all you need? \citet{disentangle}: VAEs with disentanglement penalty in addition to a reconstruction loss provide an alternative to concept bottleneck models. With traditional VAEs, there is an infinite number of latent space representations. Somewhere in the middle is "weakly-supervised VAEs" (WVAEs) which leverage concept labels to add a concept loss penalty in addition to the disentanglement loss. The authors implemented and compared VAEs, WVAEs, CMBS, and CMEs. They find that VAEs and CMEs are concept-label efficient (as they don't require concepts), CBMs and WVAEs are insensitive to downstream tasks, and CBMs and CMEs avoid "concept bias", in which concepts with higher variance are learned more accurately. They find no framework provides all three attributes. 

\item Concept-based Model Extraction \citet{cme}: Instead of training models using concepts, CMEs use concepts to analyze models -- the authors argue that in some cases retraining using concept labels may be unnecessary. 

\item On The Quality Assurance of Concept-Based Representations (submitted to ICLR 2022) \citet{zarlenga2022on}: Connects supervised concept learning (e.g., concept bottlenecks) and unsupervised disentanglement (e.g., VAEs) with evaluation metrics in terms of concept representation quality. See Reviewer yfkD on OpenReview.

\item Towards Robust Interpretability with Self-Explaining Neural Networks \citet{self_explaining}: Proposes complex interpretable models as an alternative to posteriori explanations of already-trained models. They enforce constraints towards interpretability, such as forcing the coefficients to vary slowly around each input, such that the model behaves like a collective of locally linear models. Specifically, they start with a linear regression model in which the coefficients can vary based on the inputs, but force the coefficients to vary similarly for similar inputs (local linearity). The network also transforms the input into a small set of interpretable basis features (unsupervised concept generation) and generates relevance scores for each concept. The concepts and relevance scores together yield explanations and, at inference time, are combined with an aggregator to yield a class label.

\item Concept Bottleneck Model With Additional Unsupervised Concepts \citet{cbm_auc}: Combines CBM with SENN (above) to use both supervised and unsupervised concepts. 
\item On Completeness-aware Concept-Based Explanations in Deep Neural Networks \citet{complete_cbm}: The authors propose a metric for concept quality called "completeness," which describes the ability to recover the prediction with similar accuracy when using the concepts alone. They also propose a concept discovery method for inferring complete, interpretable concepts from a training NN. The combine these for ConceptSHAP, which assigns an importance score to the learned concepts. 

\end{itemize}


\subsection{Uncertainty Quantification}
\begin{itemize}             
    \item The traditional methods for measuring uncertainty quality are ECE and OOD performance.
    \item Bayesian neural networks (BNN) and deep ensembles are the principled approaches to estimating the predictive uncertainty of a deep learning model.

    \item Ensembling: instead of finding a single set of parameters $\theta$ for the model, we can estimate a full distribution of $p(\theta|x,y)$ by obtaining multiple good settings of $\theta$. Ensembling approaches include bagging, boosting, decision trees, stacking, etc, and the uncertainty can be quantified using the standard deviation of the predictions from the models. The main downside is needing to train multiple models.
    
    \item Bayesian NNs treat inputs as RVs and attach a probability distribution to the network parameters. They can be used to prevent overfitting and allow for predictions with error metrics for OOD samples and uncertainty quantification. They are also difficult to scale. The introduced stochasticity means BNNs can be considered a special case of ensemble learning. 
    \item On Calibration of Modern Neural Networks \citet{calibrate_nn}: Modern NNs are poorly calibrated -- the authors investigate post-processing calibration methods and find "Platt scaling" after training can calibrate the system. 
    \item Does Your Dermatology Classifier Know What It Doesn’t Know? \citet{derm_uncertainty}: The authors frame infrequent conditions as OOD or 'outlier' conditions that are seen rarely or not at all during training. They assign abstention classes for each outlier class and perform course inlier vs outlier detection followed by fine-grained classification. This method performs better than those that simply using the outlier data during training, and gets better using recent representation learning methods.
    \item Simple and Principled Uncertainty Estimation with Deterministic Deep Learning via Distance Awareness \citet{uncertainty_distance}: The authors formalize uncertainty quantification as a minimax learning problem and identify the model's ability to quantify the distance of a test sample from the training data in the input space. 
    \item In practice, models assign high confidence predictions to out-of-distribution inputs \citet{uncertainty_distance}.
    \item Selective classification can  be considered by considering the respective costs of misclassification and abstaining \citet{reject_or_not, 1995_reject}. In this case, a threshold on the maximal activation in the softmax layer is selected. 
    \item A review of uncertainty quantification in deep learning \cite{abdar_uq_review}: The inherent irreducible data uncertainty (aleatoric uncertainty) is easier to quantify than knowledge uncertainty (epistemic uncertainty). 
    \item Dropout as a Bayesian Approximation \cite{dropout_uncertainty}: 
    \item \citet{freund_gen_bounds}: 
    \item Selective Classification for Deep Neural Networks \citet{selective_class}: The authors propose a method for creating a selective classifier from a trained NN, also known as selection prediction or prediction with a reject option. The goal is to equip the user with a "dial" that allows for precise control of the desired true error rate (with high probability) with tradeoff in respect to the coverage. In this work, the authors devise a method using either softmax thresholds or MC-dropout which chooses an rejection threshold given a classifier, a confidence level, and a desired risk. 
\end{itemize}

\subsection{Human in the Loop}
\begin{itemize}
    \item Soliciting human-in-the-loop user feedback for interactive machine learning reduces user trust and impressions of model accuracy \cite{honeycutt2020soliciting}. Found that providing human-in-the-loop feedback lowered both participants’ trust in the system and their perception of system accuracy, regardless of whether the system accuracy improved in response to their feedback.
    \item Perspectives on Incorporating Expert Feedback into Model Updates \cite{chen2022perspectives}
\end{itemize}


\subsection{Repairing/Debugging Neural Networks}
\begin{itemize}
    \item MODE: automated neural network model debugging via state differential analysis and input selection \cite{10.1145/3236024.3236082}: Artificial intelligence models are becoming an integral part of modern computing systems. Just like software inevitably has bugs, models have bugs too, leading to poor classification/prediction accuracy. Unlike software bugs, model bugs cannot be easily fixed by directly modifying models. Existing solutions work by providing additional training inputs. However, they have limited effectiveness due to the lack of understanding of model misbehaviors and hence the incapability of selecting proper inputs. Inspired by software debugging, we propose a novel model debugging technique that works by first conducting model state differential analysis to identify the internal features of the model that are responsible for model bugs and then performing training input selection that is similar to program input selection in regression testing. Our evaluation results on 29 different models for 6 different applications show that our technique can fix model bugs effectively and efficiently without introducing new bugs. For simple applications (e.g., digit recognition), MODE improves the test accuracy from 75\% to 93\% on average whereas the state-of-the-art can only improve to 85\% with 11 times more training time. For complex applications and models (e.g., object recognition), MODE is able to improve the accuracy from 75\% to over 91\% in minutes to a few hours, whereas state-of-the-art fails to fix the bug or even degrades the test accuracy.
    
    \item DeltaGrad: Rapid retraining of machine learning models \cite{pmlr-v119-wu20b} Machine learning models are not static and may need to be retrained on slightly changed datasets, for instance, with the addition or deletion of a set of data points. This has many applications, including privacy, robustness, bias reduction, and uncertainty quantifcation. However, it is expensive to retrain models from scratch. To address this problem, we propose the DeltaGrad algorithm for rapid retraining machine learning models based on information cached during the training phase. We provide both theoretical and empirical support for the effectiveness of DeltaGrad, and show that it compares favorably to the state of the art.
    
\end{itemize}



\iftoggle{workingversion}{
\clearpage
}{
}
\section*{Misc Notes}

\begin{itemize}
\item ``Noisy-OR works by assuming there is a disjunctive interaction among the parents of a node, rather than a conjunctive interaction. This assumption is usually interpreted in the context of a cause and effect model where each parent node is seen as an event sufficient to cause behavior in the child node. For this reason, the Noisy-OR model requires only that a node be parameterized for the instances where a single parent event occurs, rather than every parent-state combination. The resulting model is linear in the size of the largest parent set rather than exponential, as is usually the case with BNs."

\item Uncertainty-aware CBMs can leverage uncertainty scores for data augmentation using generative modeling. For example, if a model is consistently uncertain about the presence of bone spurs, we can use generative modeling to construct images with and without bone spurs, for which other concepts are held constant. More concretely, we can construct a density map of the manifold using the uncertainty metrics, and generate samples at areas of low density.


\item A common criticism relies on the choice of concepts -- what if the set of concepts is wrong/irrelevant for prediction? What if the set of concepts is the wrong size, either for prediction or for interpretability purposes?

\item The reject mechanism in our case might make sense to be based on the combinatorial confidence levels of the concepts -- how many concepts do we need to know (and with how much certainty) in order to make a reasonable prediction?

d
\item In some cases it makes sense to have different concepts for different classes \citet{complete_cbm}

\item The ability to detect mistakes in a CBM can be used for more than just intervention -- it can be used to improve the system (efficiently). We describe how to use correction from concepts and labels to improve performance and/or selective prediction bounds.

\end{itemize}

There are three types of mistakes a concept bottleneck model can make
%
\begin{itemize}
    \item Concepts are correct, but the label is wrong
    \item One or more concepts are incorrect, and the corrected concept yields the correct label
    \item One or more concepts are incorrect, but the corrected concepts don't yield the correct label
\end{itemize}
%
Each of these mistakes can be used to improve the overall performance, as we can update the model to get fewer samples like this one wrong. Specifically, we can adjust the parameters of the relevant part of the system (concept detectors vs front end) to get this point right in the future. This could include performing a careful iteration of backpropagation (e.g., principled limitation of the parameter magnitude updates) or by enforcing a constraint on the front-end (e.g., ?). 

We investigate conformal prediction in the context of CBMs to choose 1) which points to offer a prediction on and 2)  which points to use to update the system. This is helpful, as we can ask for human intervention according to our uncertainty metrics; \emph{we should prioritize repairs using samples for which the model is ``confidently wrong."} This is also a difficult and interesting problem because conformal prediction with multiple models is usually used when all models are predicting the same label. It's a different (and harder) problem when the models are predicting different labels, each of which may have class-dependent relevance to the overall label.

The architecture is the following:
    \begin{enumerate}
        \item predict concepts $\hat{\ctrue}_i$
        \item OOD detection on $\hat{\ctrue}_i$
        \item if $\hat{\ctrue}_i$ is not OOD, predict $\hat{y}_i$
        \item if $\hat{\ctrue}_i$ is OOD, i.e.,  $\hat{\ctrue}_i$ has never been seen before, then abstain. (e.g., solicit human for ground-truth label $y_i$.)
        \item if $\hat{y}_i \neq {y}_i$, repair accordingly.
    \end{enumerate}

\textbf{Hypothesis:} Repairing using ``confidently wrong" samples will be more effective than repairing using uncertain samples or a random selection of all wrong samples. \\
\\

\subsection{Datasets}

\begin{table}[!b]
\begin{tabular}{lllllll}
& Description & Concepts & Label & Num. Samples & Notes & Links \\
\begin{tabular}[c]{@{}l@{}}Forgery \\ Detection\end{tabular}            & \begin{tabular}[c]{@{}l@{}}Images of text, \\ where some\\ words are "forged" \\ (copied and pasted \\ from another\\ text image)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Font, font size, \\ character width, color,\\ blur level, etc\end{tabular}   & \begin{tabular}[c]{@{}l@{}}Vector of \\ binary labels \\ marking \\ each word\\ as "forged" \\ or "original"\end{tabular} & \begin{tabular}[c]{@{}l@{}}infinite \\ (synthetic dataset)\end{tabular}                       &                                                                                                                                           &                                                                                                                                                                                     \\
\begin{tabular}[c]{@{}l@{}}Car \\ Prices\end{tabular}                   & Images of cars                                                                                                                                 & \begin{tabular}[c]{@{}l@{}}Color, Make, Model, \\ Year, Type (sedan\\ truck, etc)\end{tabular}          & Price                                                                                                                     & \begin{tabular}[c]{@{}l@{}}TBD \\ (Kelley Blue Book?)\end{tabular}                            &                                                                                                                                           &                                                                                                                                                                                     \\
CheXpert                                                                & \begin{tabular}[c]{@{}l@{}}Chest xrays with their\\ associated radiology\\ reports\end{tabular}                                                & \begin{tabular}[c]{@{}l@{}}14 observations \\ (fracture, lung opacity, \\ support devices)\end{tabular} & \begin{tabular}[c]{@{}l@{}}5 binary \\ multiclass\\ (cardiomegaly, \\ edema, etc)\end{tabular}                            & \begin{tabular}[c]{@{}l@{}}224,316 chest \\ radiographs \\ of 65,240 \\ patients\end{tabular} & \begin{tabular}[c]{@{}l@{}}Top model \\ achieves 0.930 AUC\end{tabular}                                                                   & \begin{tabular}[c]{@{}l@{}}https://stanfordmlgroup.github.io/competitions/chexpert/\\ (scroll to bottom)\end{tabular}                                                               \\
\begin{tabular}[c]{@{}l@{}}X-ray \\ grading \\ (OAI)\end{tabular}       & \begin{tabular}[c]{@{}l@{}}Knee Xray images\\ one observation \\ is one knee \\ from one patient at\\ one of five \\ time points\end{tabular}  & \begin{tabular}[c]{@{}l@{}}10 ordinal variables \\ (bone spurs, \\ joint narrowing, etc)\end{tabular}   & \begin{tabular}[c]{@{}l@{}}0,1,2,3 \\ (osteoarthritis \\ severity)\end{tabular}                                           & 36,369                                                                                        & \begin{tabular}[c]{@{}l@{}}"Data was processed \\ on a computer with\\  several terabytes of\\ RAM and hundreds \\ of cores"\end{tabular} & \begin{tabular}[c]{@{}l@{}}https://nda.nih.gov/oai/\\ \\ https://github.com/epierson9/pain-disparities\\ \\ \textbackslash{}citet\{pierson2021algorithmic\}\end{tabular}            \\
\begin{tabular}[c]{@{}l@{}}Bird \\ identification \\ (CUB)\end{tabular} & Bird images                                                                                                                                    & \begin{tabular}[c]{@{}l@{}}312 binary concepts \\ (wing color, \\ beak shape, etc)\end{tabular}         & \begin{tabular}[c]{@{}l@{}}1 of 200 \\ bird species\end{tabular}                                                          & 11,788                                                                                        &                                                                                                                                           & \begin{tabular}[c]{@{}l@{}}http://www.vision.caltech.edu/datasets/cub\_200\_2011/\\ \\ Potential processing example: \\ https://github.com/halwai/bird\_classification\end{tabular}
\end{tabular}
\caption{Potential Datasets}
\end{table}

% \begin{itemize}
%     \item Forgery
%     \item PLCO <- \href{https://cdas.cancer.gov/learn/plco/images/}{https://cdas.cancer.gov/learn/plco/images/}
%     \item Car Prices
%     \item OpenAI LLM - what do we need to generate our own concept bottleneck dataset?
%     \item CheXpert https://stanfordmlgroup.github.io/competitions/chexpert/
%     \item Sentiment Analysis?
%     \item Breastcancer?
%     \item https://zitniklab.hms.harvard.edu/data/
% \end{itemize}



==> results/baselines.tex <==
\begin{table}
\caption{x0, ... xn $\sim$ Bernoulli(0.5)\\ c1 = parity(x0, x1, x3) w/ p=1.0\\ c2 = parity(x0, x1, x2) w/ p=1.0\\ c3 = parity(x0, x1, x4) w/ p=1.0\\ p = logistic(1.0c0 + 2.0c1 + 3.0c2 + (-2.0))\\ y $\sim$ Bernoulli(p)}
\begin{tabular}{lrrrrrr}
 & x->y LR & c->y LR & x->y MLP & x->c1 MLP & x->c2 MLP & x->c3 MLP \\
train logloss & 0.645141 & 0.434723 & 0.673571 & 0.321308 & 0.198866 & 0.230758 \\
train acc & 0.653100 & 0.795300 & 0.623800 & 1.000000 & 1.000000 & 1.000000 \\
val logloss & 0.645141 & 0.434723 & 0.673571 & 0.321308 & 0.198866 & 0.230758 \\
val acc & 0.653100 & 0.795300 & 0.623800 & 1.000000 & 1.000000 & 1.000000 \\
\end{tabular}
\end{table}
c->y LR coefficients: [[1.03728345 1.99327405 2.92621853]], INTERCEPT: [-1.9670535]

==> results/baselines_2.tex <==
\begin{table}
\caption{x0, ... xn $\sim$ Bernoulli(0.5)\\ c1 = parity(x0, x1, x3) w/ p=0.95\\ c2 = parity(x0, x1, x2) w/ p=0.95\\ c3 = parity(x0, x1, x4) w/ p=0.95\\ p = logistic(1.0c0 + 2.0c1 + 3.0c2 + (-2.0))\\ y $\sim$ Bernoulli(p)}
\begin{tabular}{lrrrrrr}
 & x->y LR & c->y LR & x->y MLP & x->c1 MLP & x->c2 MLP & x->c3 MLP \\
train logloss & 0.653548 & 0.435340 & 0.464209 & 0.116450 & 0.117555 & 0.120296 \\
train acc & 0.640490 & 0.796960 & 0.783310 & 0.975480 & 0.974970 & 0.974210 \\
val logloss & 0.651182 & 0.427912 & 0.458654 & 0.107808 & 0.119525 & 0.124455 \\
val acc & 0.643000 & 0.797000 & 0.795000 & 0.978000 & 0.975000 & 0.973000 \\
\end{tabular}
\end{table}
c->y LR coefficients: [[0.99271268 1.98510907 2.95745168]], intercept: [-1.99704621]

==> sections/problem_statement.tex <==



==> sections/related_work_notes.tex <==


\section{Related Work}

\subsection{Selective Classification}
\begin{itemize}

\item \cite{geifman2017selective}: Considers risk and abstention rate tradeoff 
$$
(f, g)(x) \triangleq \begin{cases}f(x), & \text { if } g(x)=1 \\ \text { don't know, } & \text { if } g(x)=0\end{cases}
$$

where $f$ is a classifier, $g$ is the rejector and $x$ is the input.

They consider risk with coverage $\phi$
$$
R(f, g) \triangleq \frac{E_P[\ell(f(x), y) g(x)]}{\phi(f, g)}
$$
\item \cite{el2010foundations}: trades off the abstention rate with accuracy (calls this "Risk-Coverage Trade-off."). Uses notation 
    $$
    (f, g)(x) \triangleq \begin{cases}\text { reject, }, & \text { w.p. } 1-g(x) \\ f(x), & \text { w.p. } g(x)\end{cases}
    $$
where $f$ is the base classifier, and $g$ is a selection function. If $g: X \rightarrow \{0,1\}$ then $g$ is deterministic, but abstention can also happen with some probability $[0,1]$, in which case $g$ is randomized. They use $\Phi(f, g) \triangleq \mathbf{E}[g(X)]$ for coverage and $R(f, g) \triangleq \frac{\mathbf{E}[\ell(f(X), Y) \cdot g(X)]}{\Phi(f, g)}$ for risk.
\item \cite{chow1970optimum}: The original selective classification paper. Introduced ``Chow's Rule'', a competitive baseline in which a sample is rejected if the confidence is lower than the cost of rejection (predict when one is $1-c$ confident): 

$$
f^*(\boldsymbol{x})= \begin{cases}{ }^{\abstain} & \max _y \eta_y(\boldsymbol{x}) \leq 1-c \\ \arg \max _y \eta_y(\boldsymbol{x}) & \text { otherwise }\end{cases}
$$
Here $f$ is the function that can yield $Y \cup \{\abstain\}$ and $\eta_y(x)$ is the probability of class $y$ given $x$, and $c$ is the cost of abstention.
\item \cite{mozannar2020consistent}: Proposed a consistent loss ($\hat{\theta} \rightarrow \theta^*$ as $n \rightarrow \infty$) for multiclass selective classification using connections with cost sensitive learning (e.g,. false negatives worse than false positives). References prior work that handles this problem for binary classification and  is applicable to the situation where the rejection cost can be
different for each x. They consider a split loss for when the model predicts vs when the expert predicts: 

$$
\begin{aligned}
L(h, r) & =\mathbb{E}_{(x, y) \sim \mathbf{P}, m \sim M \mid(x, y)}[\underbrace{l(x, y, h(x))}_{\text {classifier cost }} \underbrace{\mathbb{I}_{r(X)=0}}_{\text {predict }} \\
& +\overbrace{l_{\exp }(x, y, m)}^{\text {expert cost }} \overbrace{\mathbb{I}_{r(x)=1}}^{\text {defer }}]
\end{aligned}
$$

The propose the following surrogate loss, using cross entropy loss and cost sensitive learning:

$$
\begin{aligned}
& \widetilde{L}_{C E}\left(g_1, \cdots, g_{K+1}, x, c(1), \cdots, c(K+1)\right)= \\
& -\sum_{i=1}^{K+1}\left(\max _{j \in[K+1]} c(j)-c(i)\right) \log \left(\frac{\exp \left(g_i(x)\right)}{\sum_k \exp \left(g_k(x)\right)}\right)
\end{aligned}
$$

\item \cite{bartlett2008classification}: Proposes a surrogate loss to solve the problem of selective classification. They use notation: 

$$
\ell_{d, \delta}(z)= \begin{cases}1 & \text { if } z<-\delta \\ d & \text { if }|z| \leq \delta \\ 0 & \text { otherwise }\end{cases}
$$

where $\delta$ is the confidence threshold, $d$ is the cost of rejection, $z$ is the decision function. 

They reformulate this as a continuous surrogate loss: 

$$
\phi_d(z)= \begin{cases}1-a z & \text { if } z<0 \\ 1-z & \text { if } 0 \leq z<1 \\ 0 & \text { otherwise }\end{cases}
$$

\item \cite{cortes2016learning}: proposes learning two functions: a classifier $h$ and a rejection function $r$, and analyzes
the approach, giving a kernel-based algorithm in the binary setting. 

$$
R(h, r)=\underset{(x, y) \sim \mathcal{D}}{\mathbb{E}}\left[1_{y h(x) \leq 0} 1_{r(x)>0}+c 1_{r(x) \leq 0}\right]
$$

\item \cite{charoenphakdee2021classification}
Also uses connections to cost-sensitive learning, and seeks a method to reject without calculating posterior class probabilities. Considers 0-1 loss with a cost of rejection:

$$
\ell_{01 c}(f(\boldsymbol{x}), y)= \begin{cases}c & f(\boldsymbol{x})=® \\ \ell_{01}(f(\boldsymbol{x}), y) & \text { otherwise }\end{cases}
$$


\item \cite{fisch2022calibrated}: Aims  to develop a new approach to selective
classification in which we propose a method for rejecting examples with “uncertain” uncertainties, using a separate selector network is trained to improve the
selective calibration error of a given base model including on OOD samples. The model is $f$, and the rejector is $g$, with loss function $\mathcal{L}$ and coverage $\psi$.

$$
(f, g)(x):= \begin{cases}f(x) & \text { if } g(x)=1 \\ \text { "abstain" } & \text { otherwise. }\end{cases}
$$

\begin{align*}
\mathcal{R}(f, g ; P) &:= \mathbb{E}[\mathcal{L}(f(X), Y) \mid g(X)=1] \\
&= \frac{\mathbb{E}[\mathcal{L}(f(X), Y) g(X)]}{\psi(f, g ; P)}
\end{align*}

\item \cite{wilder2020learning}:
End-to-end joint learning for human-AI teamwork, electing some examples to be sent to an expert and others to model. Learns a model with the mixtures
of expert loss and explores training jointly and separately.

\item \cite{narasimhan2022post}: Shows that existing selective classification losses can underfit when there's a non-trivial deferral cost and proposes post-hoc estimators that fit a deferral function on top of a base model with threshold correction. 




\end{itemize}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=.5\textwidth]{figures/aleatoric_epistemic.png}
%     \caption{The irreducible uncertainty in data that gives rise to uncertainty in predictions is aleatoric uncertainty (also known as data uncertainty). This type of uncertainty is not a property of the model, but rather is an inherent property of the data distribution, and hence, it is irreducible. In contrast, epistemic uncertainty (also known as knowledge uncertainty) occurs due to inadequate knowledge. One can define models to answer different questions in model-based prediction. For data-rich problems, there may be massive collections of data that are information poor. In such cases, AI-based methods can be used to define the efficient models that characterize the emergent features of the data. Very often, the data in hand are incomplete, noisy, discordant or multimodal}
%     \label{fig:aleatoric_epistemic}
% \end{figure}




\subsection{Concept Bottleneck Models}
\begin{itemize}

\item \cite{chauhan2022interactive}: Combines concept prediction uncertainty and influence to choose with the goal of 
maximally improving the final prediction. Uses a greedy algorithm to intervene on concepts up to a budget $B$.


\begin{algorithm}
\caption{Policy Rollout}
\label{algo:policy_rollout}
\begin{algorithmic}[1]
\REQUIRE $B$, $q_i$, $x$
\ENSURE Prediction $\operatorname{argmax}_{y \in \mathcal{Y}} p_\phi(c_S, p_\theta(c_{\bar{S}} \mid x))$
\STATE $S \gets \emptyset$
\STATE $b \gets 0$
\WHILE{$b \leq B$}
    \STATE $i \gets \psi(S)$
    \IF{$b \leq B-q_i$}
        \STATE Acquire the label for concept $c_i$
        \STATE $S \gets S \cup \{i\}$
        \STATE $b \gets b+q_i$
    \ELSE
        \STATE $b \gets B+1$
    \ENDIF
\ENDWHILE
\STATE Output prediction $\operatorname{argmax}_{y \in \mathcal{Y}} p_\phi(c_S, p_\theta(c_{\bar{S}} \mid x))$
\end{algorithmic}
\end{algorithm}

The interventions are determined by simply scoring the uncertainty and the concept importance: 

\begin{algorithm}
\caption{CooP policy}
\label{algo:coop_policy}
\begin{algorithmic}[1]
\STATE \textbf{Given} $p_\theta$, $p_\phi$, $q$, set of concepts acquired so far $S$, highest scoring predicted label based on acquired concepts $k \in \mathcal{Y}$, and score importance weights $\alpha$, $\beta$, $\gamma \in \mathbb{R}_+$.
\FORALL{$i \in \bar{S}$}
    \STATE Compute score$_i = \alpha \operatorname{CPU}(c_i ; S) + \beta \operatorname{CIS}(c_i ; S, k) - \gamma q_i$
\ENDFOR
\STATE \textbf{Output} $\operatorname{argmax}_i$ score$_i$
\end{algorithmic}
\end{algorithm}






\item Concept Bottlenecks \citet{koh2020concept}: Concept bottlenecks can be useful for understanding which important features the model might have learned (“Did the model deem the space between the knee joints too narrow?”) as well as for improving performance through concept correction (“If the radiologist informed the model the x-ray shows a bone spur, would its prediction change?”). They present weak evidence that CBMs require less data for similar performance and may be more robust to covariate shift.

\item Do Concept Bottleneck Models Learn as Intended? \citet{cbm_work}: The authors claim that of the three proposed training methods (independent, joint, and sequential), only the independent method may be able to achieve interpretability (which concepts are important), predictability (predict targets from concepts alone), and intervenability (fix concepts to improve performance). First, they use an ablation study to demonstrate that the joint model is learning labels before the concept to label component. This finding means that there's not a clear relationship between concepts and labels and that it may not be possible to predict labels from concepts alone. Second, They use Integrated Gradients, Gradient, and SmoothGrad to demonstrate that the model may be using other parts of the image to learn concepts (using the whole bird to learn wing color). Note: This experiment is perhaps poorly motivated since even humans use other parts of an image for concept learning (e.g., it can be difficult to determine if you're looking at a wing without looking at the rest of the image) and the examples were cherry-picked. 

\item Is Disentanglement all you need? \citet{disentangle}: VAEs with disentanglement penalty in addition to a reconstruction loss provide an alternative to concept bottleneck models. With traditional VAEs, there is an infinite number of latent space representations. Somewhere in the middle is "weakly-supervised VAEs" (WVAEs) which leverage concept labels to add a concept loss penalty in addition to the disentanglement loss. The authors implemented and compared VAEs, WVAEs, CMBS, and CMEs. They find that VAEs and CMEs are concept-label efficient (as they don't require concepts), CBMs and WVAEs are insensitive to downstream tasks, and CBMs and CMEs avoid "concept bias", in which concepts with higher variance are learned more accurately. They find no framework provides all three attributes. 

\item Concept-based Model Extraction \citet{cme}: Instead of training models using concepts, CMEs use concepts to analyze models -- the authors argue that in some cases retraining using concept labels may be unnecessary. 

\item On The Quality Assurance of Concept-Based Representations (submitted to ICLR 2022) \citet{zarlenga2022on}: Connects supervised concept learning (e.g., concept bottlenecks) and unsupervised disentanglement (e.g., VAEs) with evaluation metrics in terms of concept representation quality. See Reviewer yfkD on OpenReview.

\item Towards Robust Interpretability with Self-Explaining Neural Networks \citet{self_explaining}: Proposes complex interpretable models as an alternative to posteriori explanations of already-trained models. They enforce constraints towards interpretability, such as forcing the coefficients to vary slowly around each input, such that the model behaves like a collective of locally linear models. Specifically, they start with a linear regression model in which the coefficients can vary based on the inputs, but force the coefficients to vary similarly for similar inputs (local linearity). The network also transforms the input into a small set of interpretable basis features (unsupervised concept generation) and generates relevance scores for each concept. The concepts and relevance scores together yield explanations and, at inference time, are combined with an aggregator to yield a class label.

\item Concept Bottleneck Model With Additional Unsupervised Concepts \citet{cbm_auc}: Combines CBM with SENN (above) to use both supervised and unsupervised concepts. 
\item On Completeness-aware Concept-Based Explanations in Deep Neural Networks \citet{complete_cbm}: The authors propose a metric for concept quality called "completeness," which describes the ability to recover the prediction with similar accuracy when using the concepts alone. They also propose a concept discovery method for inferring complete, interpretable concepts from a training NN. The combine these for ConceptSHAP, which assigns an importance score to the learned concepts. 

\end{itemize}


\subsection{Uncertainty Quantification}
\begin{itemize}             
    \item The traditional methods for measuring uncertainty quality are ECE and OOD performance.
    \item Bayesian neural networks (BNN) and deep ensembles are the principled approaches to estimating the predictive uncertainty of a deep learning model.

    \item Ensembling: instead of finding a single set of parameters $\theta$ for the model, we can estimate a full distribution of $p(\theta|x,y)$ by obtaining multiple good settings of $\theta$. Ensembling approaches include bagging, boosting, decision trees, stacking, etc, and the uncertainty can be quantified using the standard deviation of the predictions from the models. The main downside is needing to train multiple models.
    
    \item Bayesian NNs treat inputs as RVs and attach a probability distribution to the network parameters. They can be used to prevent overfitting and allow for predictions with error metrics for OOD samples and uncertainty quantification. They are also difficult to scale. The introduced stochasticity means BNNs can be considered a special case of ensemble learning. 
    \item On Calibration of Modern Neural Networks \citet{calibrate_nn}: Modern NNs are poorly calibrated -- the authors investigate post-processing calibration methods and find "Platt scaling" after training can calibrate the system. 
    \item Does Your Dermatology Classifier Know What It Doesn’t Know? \citet{derm_uncertainty}: The authors frame infrequent conditions as OOD or 'outlier' conditions that are seen rarely or not at all during training. They assign abstention classes for each outlier class and perform course inlier vs outlier detection followed by fine-grained classification. This method performs better than those that simply using the outlier data during training, and gets better using recent representation learning methods.
    \item Simple and Principled Uncertainty Estimation with Deterministic Deep Learning via Distance Awareness \citet{uncertainty_distance}: The authors formalize uncertainty quantification as a minimax learning problem and identify the model's ability to quantify the distance of a test sample from the training data in the input space. 
    \item In practice, models assign high confidence predictions to out-of-distribution inputs \citet{uncertainty_distance}.
    \item Selective classification can  be considered by considering the respective costs of misclassification and abstaining \citet{reject_or_not, 1995_reject}. In this case, a threshold on the maximal activation in the softmax layer is selected. 
    \item A review of uncertainty quantification in deep learning \cite{abdar_uq_review}: The inherent irreducible data uncertainty (aleatoric uncertainty) is easier to quantify than knowledge uncertainty (epistemic uncertainty). 
    \item Dropout as a Bayesian Approximation \cite{dropout_uncertainty}: 
    \item \citet{freund_gen_bounds}: 
    \item Selective Classification for Deep Neural Networks \citet{selective_class}: The authors propose a method for creating a selective classifier from a trained NN, also known as selection prediction or prediction with a reject option. The goal is to equip the user with a "dial" that allows for precise control of the desired true error rate (with high probability) with tradeoff in respect to the coverage. In this work, the authors devise a method using either softmax thresholds or MC-dropout which chooses an rejection threshold given a classifier, a confidence level, and a desired risk. 
\end{itemize}

\subsection{Human in the Loop}
\begin{itemize}
    \item Soliciting human-in-the-loop user feedback for interactive machine learning reduces user trust and impressions of model accuracy \cite{honeycutt2020soliciting}. Found that providing human-in-the-loop feedback lowered both participants’ trust in the system and their perception of system accuracy, regardless of whether the system accuracy improved in response to their feedback.
    \item Perspectives on Incorporating Expert Feedback into Model Updates \cite{chen2022perspectives}
\end{itemize}


\subsection{Repairing/Debugging Neural Networks}
\begin{itemize}
    \item MODE: automated neural network model debugging via state differential analysis and input selection \cite{10.1145/3236024.3236082}: Artificial intelligence models are becoming an integral part of modern computing systems. Just like software inevitably has bugs, models have bugs too, leading to poor classification/prediction accuracy. Unlike software bugs, model bugs cannot be easily fixed by directly modifying models. Existing solutions work by providing additional training inputs. However, they have limited effectiveness due to the lack of understanding of model misbehaviors and hence the incapability of selecting proper inputs. Inspired by software debugging, we propose a novel model debugging technique that works by first conducting model state differential analysis to identify the internal features of the model that are responsible for model bugs and then performing training input selection that is similar to program input selection in regression testing. Our evaluation results on 29 different models for 6 different applications show that our technique can fix model bugs effectively and efficiently without introducing new bugs. For simple applications (e.g., digit recognition), MODE improves the test accuracy from 75\% to 93\% on average whereas the state-of-the-art can only improve to 85\% with 11 times more training time. For complex applications and models (e.g., object recognition), MODE is able to improve the accuracy from 75\% to over 91\% in minutes to a few hours, whereas state-of-the-art fails to fix the bug or even degrades the test accuracy.
    
    \item DeltaGrad: Rapid retraining of machine learning models \cite{pmlr-v119-wu20b} Machine learning models are not static and may need to be retrained on slightly changed datasets, for instance, with the addition or deletion of a set of data points. This has many applications, including privacy, robustness, bias reduction, and uncertainty quantifcation. However, it is expensive to retrain models from scratch. To address this problem, we propose the DeltaGrad algorithm for rapid retraining machine learning models based on information cached during the training phase. We provide both theoretical and empirical support for the effectiveness of DeltaGrad, and show that it compares favorably to the state of the art.
    
\end{itemize}


==> shortcuts.tex <==

\usepackage{pgffor}

%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%  editing shortcuts  %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\todo}[1]{{\large \textcolor{red}{[TODO: #1]}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%  common math functions  %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% arg functions
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\minimize}{minimize}
\DeclareMathOperator*{\maximize}{maximize}


% indicator functions
\newcommand{\indic}{\mathds{1}}
\newcommand{\indicarg}[1]{\mathds{1}\left\{ #1 \right\}}
\newcommand{\indicsarg}[2]{\mathds{1}_{#1}\left\{ #2 \right\}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%  probability & statistics  %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% probability functions
\newcommand{\Parg}[1]{\mathbb{P}\left( #1 \right)}
\newcommand{\Psarg}[2]{\mathbb{P}_{#1}\left( #2 \right)}
\newcommand{\Earg}[1]{\mathbb{E} \, \left[ #1 \right]}
\newcommand{\Esarg}[2]{\mathbb{E}_{#1} \, \left[ #2 \right]}
\newcommand{\Vararg}[1]{\mathrm{Var} \, \left[ #1 \right]}
\newcommand{\Varsarg}[2]{\mathrm{Var}_{#1} \,  \left[ #2  \right]}
\newcommand{\cov}{\mathrm{Cov}}


% distributions
\newcommand{\Uniform}{\mathrm{Unif}}
\newcommand{\Poisson}{\mathrm{Pois}}
\newcommand{\Geometric}{\mathrm{Geo}}
\newcommand{\Exponential}{\mathrm{Expo}}
\newcommand{\Bernoulli}{\mathrm{Bern}}
\newcommand{\Normal}{\mathcal{N}}
\newcommand{\Binomial}{\mathrm{Binomial}}

\newcommand{\GP}{\Gc\Pc}

\newcommand{\simiid}{\overset{iid}{\sim}}
\newcommand{\simind}{\overset{ind}{\sim}}
\newcommand{\iid}{i.i.d.\ }
\newcommand{\eqdist}{\overset{\textrm{dist}}{=}}


%%%%%%%%%%%%%%%%%%%%%%%%
%%%  font shortcuts  %%%
%%%%%%%%%%%%%%%%%%%%%%%%

%% UPPER CASE FONTS %%%%%%%%%%%%%%%%%%%%%%
\foreach \x in {A,...,Z}{
% mathcal
\expandafter\xdef\csname 
\x c%
\endcsname{\noexpand\ensuremath{\noexpand\mathcal{\x}}}
% tilde
\expandafter\xdef\csname 
\x til%
\endcsname{\noexpand\ensuremath{\noexpand\tilde{\x}}}
% mathbb
\expandafter\xdef\csname 
\x bb%
\endcsname{\noexpand\ensuremath{\noexpand\mathbb{\x}}}
% mathbf
\expandafter\xdef\csname 
\x b%
\endcsname{\noexpand\ensuremath{\noexpand\mathbf{\x}}}
% hat
\expandafter\xdef\csname 
\x h%
\endcsname{\noexpand\ensuremath{\noexpand\hat{\x}}}
% widehat
\expandafter\xdef\csname 
\x wh%
\endcsname{\noexpand\ensuremath{\noexpand\widehat{\x}}}
}

%% LOWER CASE FONTS %%%%%%%%%%%%%%%%%%%%%%
\foreach \x in {a,...,z}{
% tilde
\expandafter\xdef\csname 
\x til%
\endcsname{\noexpand\ensuremath{\noexpand\tilde{\x}}}
% mathbf
\expandafter\xdef\csname 
\x b%
\endcsname{\noexpand\ensuremath{\noexpand\mathbf{\x}}}
% hat
\expandafter\xdef\csname 
\x h%
\endcsname{\noexpand\ensuremath{\noexpand\hat{\x}}}
% widehat
\expandafter\xdef\csname 
\x wh%
\endcsname{\noexpand\ensuremath{\noexpand\widehat{\x}}}
}

%% GREEK FONTS %%%%%%%%%%%%%%%%%%%%%%
\newcommand{\eps}{\epsilon}
\newcommand{\ve}{\varepsilon}
\newcommand{\vt}{\vartheta}
\newcommand{\vr}{\varrho}
\newcommand{\vp}{\varphi}

\edef \greek {alpha, beta, gamma, Gamma, delta, Delta, eps, ve, zeta, eta, theta, Theta, vt, iota, kappa, lambda, Lambda, mu, nu, xi, Xi, pi, Pi, rho, vr, sigma, Sigma, tau, upsilon, Upsilon, phi, vp, Phi, chi, psi, Psi, omega, Omega}

\foreach \x in \greek {
% hat
\expandafter\xdef\csname 
\x h%
\endcsname{\noexpand\ensuremath{\noexpand\hat{ {\csname \x \endcsname}}}}
%
% widehat
\expandafter\xdef\csname 
\x wh%
\endcsname{\noexpand\ensuremath{\noexpand\widehat{ {\csname \x \endcsname}}}}
%
% tilde
\expandafter\xdef\csname 
\x til%
\endcsname{\noexpand\ensuremath{\noexpand\tilde{ {\csname \x \endcsname}}}}
}

%% COLORS %%%%%%%%%%%%%%%%%%%%%%
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\green}[1]{\textcolor{green}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\purple}[1]{\textcolor{purple}{#1}}
\newcommand{\orange}[1]{\textcolor{orange}{#1}}
\newcommand{\yellow}[1]{\textcolor{yellow}{#1}}
\newcommand{\gray}[1]{\textcolor{gray}{#1}}

%%%%%%%%%%%%%%%%%%%%%%%%
%%%  bracket size shortcuts  %%%
%%%%%%%%%%%%%%%%%%%%%%%%

% left / right shortcuts
\newcommand{\lrs}[1]{\left[ #1 \right]}
\newcommand{\lrp}[1]{\left( #1 \right)}
\newcommand{\lrb}[1]{\left\{ #1 \right\}}
\newcommand{\set}[1]{\left\{ #1 \right\}}
\newcommand{\lrv}[1]{\left\vert #1 \right\vert}
\newcommand{\lrn}[1]{\left\Vert #1 \right\Vert}
\newcommand{\lra}[1]{\left\langle #1 \right\rangle}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%  symbols and decorations  %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% variables
\newcommand{\Yhat}{\widehat{Y}}
\newcommand{\yhat}{\widehat{y}}
\newcommand{\ybar}{\overline{y}}
\newcommand{\ytil}{\tilde{y}}
\newcommand{\ve}{\varepsilon}
\newcommand{\vp}{\varphi}

% punctuation
\newcommand{\midc}{ \, \, {:} \, \, }
\newcommand{\midsc}{ \, \, {;} \, \, }


% independence symbol
\newcommand{\indep}{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern3mu{#1#2}}}



